Ground truth clustering is not the optimum clustering

The clustering of data is one of the most important and challenging topics in data science. The minimum sum-of-squares clustering (MSSC) problem asks to cluster the data points into $k$ clusters such that the sum of squared distances between the data points and their cluster centers (centroids) is minimized. This problem is NP-hard, but there exist exact solvers that can solve such problem to optimality for small or medium size instances. In this paper, we use a branch-and-bound solver based on semidefinite programming relaxations called SOS-SDP to compute the optimum solutions of the MSSC problem for various $k$ and for multiple datasets, with real and artificial data, for which the data provider has provided ground truth clustering. Next, we use several extrinsic and intrinsic measures to evaluate how the optimum clustering and ground truth clustering matches, and how well these clusterings perform with respect to the criteria underlying the intrinsic measures. Our calculations show that the ground truth clusterings are generally far from the optimum solution to the MSSC problem. Moreover, the intrinsic measures evaluated on the ground truth clusterings are generally significantly worse compared to the optimum clusterings. However, when the ground truth clustering is in the form of convex sets, e.g., ellipsoids, that are well separated from each other, the ground truth clustering comes very close to the optimum clustering.

==> Exact clustering with SOS-SDPA_arxiv/artificial_data_summary.tex <==
name,type,n,m,K, M
3-spiral,artificial,312,3,3, numerical
3MC,artificial,400,3,3, numerical
blobs,artificial,300,3,3, numerical
flame,artificial,240,3,3, numerical
gaussians1,artificial,100,3,2, numerical
insect,artificial,30,4,3, numerical
jain,artificial,373,3,2, numerical
lsun,artificial,400,3,3, numerical
pathbased,artificial,300,3,3, numerical
zelnik1,artificial,299,3,3, numerical
zelnik2,artificial,303,3,3, numerical
zelnik6,artificial,238,3,3, numerical

==> Exact clustering with SOS-SDPA_arxiv/artificial_data_summary_all_label_clust_eval.tex <==
dataname,k,opt_sos_sdp,normalized_mutual_info_score,mutual_info_score,homogeneity_score,fowlkes_mallows_score,completeness_score,adjusted_rand_score,adjusted_mutual_info_score,calinski_harabasz_score,davies_bouldin_score,silhouette_score
3-spiral,3.0,30109.350350293127,1.0,1.09839564632427,1.0,1.0,1.0,1.0,1.0,5.797852185441633,5.882022552277643,0.0013442973442779
3-spiral,2.0,19577.3,0.0009328955978473,0.0008355749515184,0.0007607231094866,0.4044833947646889,0.0012058015309933,-0.0031886440583456,-0.0026783716457486,184.66433452888432,1.168152962826578,0.3480876615461452
3-spiral,3.0,12286.9,0.0005112830235959,0.0005614493915305,0.0005111540576561,0.3275926899333746,0.0005114120546293,-0.005874151386097,-0.0054089048486768,238.3129233311469,0.884839446512841,0.3602912839819129
3-spiral,4.0,9200.4,0.0026194124162049,0.003254053151893,0.0029625510286594,0.2827842205353122,0.0023475110462869,-0.0050653629758994,-0.0052464948632868,245.93028258579045,0.8785236009097113,0.3543972875897688
3-spiral,5.0,7352.09,0.0064345040046559,0.0086788750617078,0.0079014106535758,0.2566357692124038,0.0054269787039899,-0.0022495671885655,-0.0032306153528088,249.36326257951583,0.889096006582799,0.3467646558672821
3MC,3.0,2056.336029450354,1.0,1.079870587934092,1.0,1.0,1.0,1.0,1.0,628.0489014193492,0.7076334829953922,0.4956142510948985
3MC,2.0,3204.77,0.4492228686363406,0.3981389737408716,0.3686913767163101,0.6126015252672271,0.5747663246293778,0.3283870126024342,0.4476566547666701,665.3804951049577,0.7242621893125113,0.5317451487655634
3MC,3.0,1929.39,0.8088691368366148,0.8788705592783972,0.8138665587325336,0.8682238227217552,0.8039327121910247,0.800264438809702,0.8079792049412197,682.4342519561616,0.7032848636744014,0.503592712829231
3MC,4.0,1221.71,0.7291369396590458,0.8957391961817014,0.8294875387756846,0.7303487823449379,0.6504465464055365,0.6070850142928569,0.727458016882152,793.1390215212372,0.7097562688818153,0.4935811979304618
3MC,5.0,786.808,0.7620462130315269,1.0156659897878242,0.9405441736596436,0.7543020207446631,0.6404925281766825,0.6365931123788192,0.7602270163151567,975.9086777188984,0.6328629570160211,0.5254332576187837
blobs,3.0,149.58362626275363,1.0,1.0986122886681091,1.0,1.0,1.0,1.0,1.0,575.4294853200782,0.607849845884483,0.5448276995403188
blobs,2.0,337.014,0.58014076123848,0.5130846366030858,0.4670297628157049,0.7178464751213609,0.7655513902623196,0.4954620872105025,0.5785408945824253,346.7956679706255,0.7930103565086946,0.4831007301050531
blobs,3.0,144.77,0.8616213640770951,0.946544591906397,0.8615820173046946,0.9351244029785276,0.8616607144434407,0.9030061261184824,0.8607687905808963,599.5022773042637,0.5937411887518809,0.559522406348139
blobs,4.0,123.004,0.7649005596468567,0.9363669477900084,0.8523179263953098,0.8378071194534666,0.6937469132566524,0.7628371840809773,0.7629400163807599,486.2641876513297,0.8445585584294051,0.4596767965245963
blobs,5.0,105.468,0.6973676167522715,0.9318293362395388,0.8481876143668774,0.7383789065439691,0.5920861543953757,0.6228084107360515,0.6942709012234543,436.1628497272959,0.977027369372981,0.3628953795527692
flame,2.0,3543.5300833896777,1.0,0.654843055442027,1.0,1.0,1.0,1.0,1.0,110.39059785543064,1.1605356766266266,0.3284556923027034
flame,2.0,3123.77,0.3987957374536851,0.2685370288304292,0.410078455591414,0.7363906803426874,0.3881172502537466,0.4534129232216995,0.3969167583837185,157.20621184586793,1.115414499722493,0.3784940710795816
flame,3.0,1913.55,0.4862702494211092,0.421887845243327,0.6442579511796879,0.7037862995686953,0.3905081610155974,0.4615695027134954,0.4837665868329622,202.7214129395292,0.799521740580789,0.4120656817418855
flame,4.0,1211.45,0.5401951313617974,0.5423000184997735,0.8281373895516299,0.6713416323651232,0.4008278323502659,0.4296731714964762,0.5372775422796912,258.16406743385016,0.6955953710582403,0.4426011973843992
gaussian1,2,0.607786784602029,1.0,0.6931471805599458,1.0,1.0,1.0,1.0,1.0,2000.6559204985397,0.19115128249343344,0.8613276990526753
gaussian1,2,0.607787,1.0,0.6931471805599458,1.0,1.0,1.0,1.0,1.0,2000.6559204985397,0.19115128249343344,0.8613276990526753
gaussian1,3,0.450486,0.8029784244290346,0.6931471805599458,1.0,0.8668497975016037,0.6708136601848828,0.7533010626414229,0.8006130337815637,1352.7850820752535,0.6940085469376062,0.6254060096221804
gaussian1,4,0.336638,0.6822742828433005,0.6931471805599457,0.9999999999999999,0.7329003050503234,0.5177665381802417,0.5396406223089729,0.6773693648790168,1205.2383930182614,0.9463542134292653,0.3791063656428615
insect,3.0,7671.200000000002,1.0,1.0986122886681096,1.0,1.0,1.0,1.0,1.0,45.770922411096016,0.8261096696425358,0.3895558522669933
insect,2.0,10683.5,0.5714653581432843,0.506210859163194,0.4607729809548126,0.6920827420915049,0.7521576281325172,0.4680581910183428,0.5532686294745759,60.27075259031997,0.5799482315693878,0.5487736943919346
insect,3.0,6002.75,0.6449126680040378,0.7053771852381958,0.6420619835714308,0.739971420144161,0.647788778776089,0.6210196944597828,0.6188196252675324,62.245133480488114,0.6953071628687374,0.4687681249232857
insect,4.0,4236.08,0.608739437554484,0.7529275783523527,0.6853442166254631,0.6024640760767093,0.5475380311755307,0.4506480558325025,0.567532700638249,60.23961599748195,0.7966716127699024,0.4367901247098583
insect,5.0,3075.25,0.6225083430893742,0.8194198139949896,0.7458680577735064,0.6125306510286749,0.5341627402160611,0.4690392923266817,0.5691211202622894,62.19958404465761,0.6300622543768848,0.494629899471638
jain,2,29856.32807886973,1.0,0.573112993765099,1.0,1.0,1.0,1.0,1.0,279.48312216168654,0.8996694938176657,0.40246004427612914
jain,2,22208.8,0.36557366684627635,0.23116584276216418,0.40335125058586924,0.6977229525630237,0.33426650953158143,0.3180937556197384,0.36421819127351646,503.4754674444723,0.783072419818396,0.49508103615678445
jain,3,12650.1,0.364735042844682,0.3039508997765924,0.5303507390048328,0.6091264821881899,0.2779408456210691,0.26254177264068607,0.36266884818536577,580.5550521784285,0.6975972408412426,0.4865910776769234
jain,4,8763.07,0.41356869205044755,0.3977188212155168,0.6939623172782735,0.5761813788589303,0.2945546646443085,0.25209632732790277,0.4110797620348116,611.7632259389032,0.792489594238666,0.47945975995143336
lsun,3.0,449.41446954502993,1.0,1.0397207708399177,1.0,1.0,1.0,1.0,1.0,384.4387306734788,0.7089983903842373,0.4774564120231758
lsun,2.0,670.265,0.6491389545399219,0.5611197584224346,0.5396831285472399,0.8181307280119151,0.8142889578784085,0.6660385013251185,0.6481154029375052,385.6928321259544,0.936232660872166,0.4606180392796291
lsun,3.0,381.646,0.5400568656616177,0.5655071130232259,0.5439028716973618,0.6423892311282245,0.5362648689101579,0.4358084271876845,0.5378309512789192,487.9512441770458,0.761378721589555,0.4967022054099482
lsun,4.0,202.504,0.7222378729708145,0.8648766312254383,0.8318354845664621,0.7254440500031895,0.6381580310742303,0.5868596025789136,0.7204692059389957,728.3004198673977,0.5579387214345408,0.5655319907213792
lsun,5.0,143.899,0.8040765861704536,1.039720770839918,1.0000000000000002,0.7712101533765884,0.6723478919069458,0.6477916751094491,0.8025284399220705,806.9620443446847,0.5826937708312114,0.5666015023842174
pathbased,3.0,22689.190096315666,1.0,1.0960106146053783,1.0,1.0,1.0,1.0,1.0,51.90716154797278,2.5279577241776545,0.260827350983948
pathbased,2.0,13638.3,0.4909971532293818,0.4392356920521657,0.4007586114577127,0.6519055872239359,0.6336831547050913,0.3989713297894657,0.4890804951430663,371.0553030050826,0.7522586238450906,0.5150123044043785
pathbased,3.0,8957.91,0.5458430500422186,0.5620602381069193,0.512823717778765,0.6616839023616249,0.5834070523255318,0.4613289348654503,0.5428393181773931,359.10473171402344,0.6692535513389878,0.5419218557223351
pathbased,4.0,7230.33,0.4658578423230228,0.5496313607454874,0.5014836110354494,0.580607790951345,0.4349580956992332,0.3827734541613792,0.4612180471591813,319.1811337346417,0.8696701159591098,0.4352170786214091
pathbased,5.0,5901.86,0.4666431283706784,0.5981987867410505,0.545796526757575,0.5838176774556085,0.4075401699442199,0.4076167756503255,0.460928129070025,308.8800396373083,0.9428932950905058,0.3825725727537546
zelnik1,3,13.50248673323875,1.0,1.0463564577282705,1.0,1.0,1.0,1.0,1.0,0.014217517052841574,120.43118334004778,-0.010563524873156782
zelnik1,2,9.60258,0.12186112054419279,0.103248340258415,0.09867415592060855,0.4602705429856286,0.15929249721219604,0.02615527060591208,0.11835050146180513,120.66118216909004,1.3011778495789665,0.30622537731244953
zelnik1,3,6.88992,0.1621105715363804,0.16899227096214928,0.16150545037878009,0.4030883988072931,0.1627202442274319,0.05330698323782812,0.15663535783669041,142.07033597185406,1.0628037616106143,0.3273632309615051
zelnik1,4,5.48487,0.2052404753362546,0.24356706913062656,0.23277638067951675,0.3881516397256538,0.1835300813021801,0.0993537434579592,0.19836296340096374,143.76413641071147,1.0732411603047478,0.32553395341276403
zelnik1,5,4.14001,0.38481469008921537,0.47284648160580967,0.4518980870366107,0.46124294710352826,0.33507365422744406,0.20297872393034727,0.37786636674666907,166.24032659730273,0.8420161038120229,0.39752307176738416
zelnik2,3,27.21008027054806,1.0,1.0975939420343654,1.0,1.0,1.0,1.0,1.0,50.53473179960157,2.2837843856324795,0.4692214114072803
zelnik2,2,18.8778,0.5035596810686214,0.4508601731442408,0.4107713753490491,0.6651722410068127,0.6504997357372246,0.42096401946901046,0.5017106628316834,279.02146941811594,0.6981217369734207,0.5749904584972232
zelnik2,3,11.8813,0.5463765765707048,0.5537671932724482,0.5045282887094413,0.6726050010685936,0.5957950174263004,0.4708785919450187,0.5433510431307448,309.2557998452903,0.6032329891280371,0.6322744873259036
zelnik2,4,8.68286,0.556547659042638,0.6040810733233957,0.550368447008504,0.6765081658527577,0.5628671996937633,0.4937406137101005,0.5523355426870863,317.88997412340456,0.5886644441624687,0.6536244570141765
zelnik2,5,6.37043,0.6113245263886611,0.7225693687305899,0.6583212070133367,0.7101001750745403,0.5705908032997264,0.5654820896922822,0.6067883724773538,350.9179183446262,0.6020361202471877,0.6824724738526461
zelnik6,3,6.0499989559164025,1.0,1.0719022217569947,1.0,1.0,1.0,1.0,1.0,191.4378235419437,1.5564445962690894,0.5749826418958833
zelnik6,2,3.80238,0.5979727711023263,0.5266688268014077,0.49134036305860557,0.7664423540430446,0.7637173981526055,0.5821826429846935,0.59602789846613,751.2905120512687,0.3519045622593329,0.7348068903877594
zelnik6,3,2.49599,0.6400618519311038,0.6248330276145528,0.5829197989629743,0.7915155418959071,0.7096244161981063,0.6483717070239138,0.636822029675717,631.3318427553139,0.5120883365552338,0.7371089795591736
zelnik6,4,1.37484,0.6733330764904996,0.7092776134836439,0.6616999191596419,0.8178682551332983,0.6853825921323213,0.705791595796343,0.6691589254118446,824.4668082737813,0.42392184952718037,0.7599966725533781
zelnik6,5,1.07112,0.6835882968102652,0.751594176677411,0.7011779259543329,0.8301868975785732,0.6668595720051071,0.7307789007864689,0.6782580684682645,806.8097010845635,0.47163075434077983,0.73735109102075



==> Exact clustering with SOS-SDPA_arxiv/artificial_data_summary_clust_eval.tex <==
dataname,k,opt_sos_sdp,true_k,normalized_mutual_info_score,mutual_info_score,homogeneity_score,fowlkes_mallows_score,completeness_score,adjusted_rand_score,adjusted_mutual_info_score,calinski_harabasz_score,davies_bouldin_score,silhouette_score,
3-spiral,2.0,19577.3,0,0.0009328955978473127,0.0008355749515184253,0.0007607231094866753,0.4044833947646889,0.001205801530993308,-0.003188644058345625,-0.0026783716457486444,184.66433452888432,1.1681529628265779,0.34808766154614523,
3-spiral,3.0,12286.9,1,0.0005112830235959982,0.0005614493915305219,0.0005111540576561699,0.3275926899333746,0.0005114120546293565,-0.005874151386097084,-0.005408904848676883,238.3129233311469,0.884839446512841,0.36029128398191296,
3-spiral,4.0,9200.4,0,0.002619412416204974,0.0032540531518930327,0.0029625510286594545,0.2827842205353122,0.002347511046286977,-0.005065362975899442,-0.005246494863286878,245.93028258579045,0.8785236009097113,0.35439728758976885,
3-spiral,5.0,7352.09,0,0.006434504004655965,0.008678875061707891,0.007901410653575825,0.25663576921240383,0.00542697870398998,-0.002249567188565553,-0.0032306153528088503,249.36326257951583,0.8890960065827991,0.34676465586728217,
3MC,2.0,3204.77,0,0.44922286863634064,0.3981389737408716,0.3686913767163101,0.6126015252672271,0.5747663246293778,0.3283870126024342,0.44765665476667016,665.3804951049577,0.7242621893125113,0.5317451487655634,
3MC,3.0,1929.39,1,0.8088691368366148,0.8788705592783972,0.8138665587325336,0.8682238227217552,0.8039327121910247,0.8002644388097021,0.8079792049412197,682.4342519561617,0.7032848636744014,0.503592712829231,
3MC,4.0,1221.71,0,0.7291369396590458,0.8957391961817014,0.8294875387756846,0.7303487823449379,0.6504465464055365,0.6070850142928569,0.727458016882152,793.1390215212372,0.7097562688818153,0.4935811979304618,
3MC,5.0,786.808,0,0.7620462130315269,1.0156659897878242,0.9405441736596436,0.7543020207446631,0.6404925281766825,0.6365931123788192,0.7602270163151567,975.9086777188983,0.6328629570160211,0.5254332576187837,
blobs,2.0,337.014,0,0.58014076123848,0.5130846366030858,0.467029762815705,0.7178464751213609,0.7655513902623196,0.4954620872105026,0.5785408945824253,346.7956679706255,0.7930103565086946,0.4831007301050532,
blobs,3.0,144.77,1,0.8616213640770951,0.9465445919063971,0.8615820173046946,0.9351244029785276,0.8616607144434407,0.9030061261184824,0.8607687905808963,599.5022773042638,0.5937411887518809,0.5595224063481391,
blobs,4.0,123.00399999999999,0,0.7649005596468567,0.9363669477900084,0.8523179263953098,0.8378071194534666,0.6937469132566524,0.7628371840809773,0.7629400163807599,486.2641876513297,0.8445585584294051,0.4596767965245963,
blobs,5.0,105.46799999999999,0,0.6973676167522715,0.9318293362395388,0.8481876143668774,0.7383789065439691,0.5920861543953757,0.6228084107360515,0.6942709012234543,436.16284972729585,0.9770273693729808,0.3628953795527693,
flame,2.0,3123.77,1,0.3987957374536851,0.2685370288304292,0.4100784555914141,0.7363906803426874,0.3881172502537466,0.4534129232216995,0.39691675838371854,157.2062118458679,1.115414499722493,0.3784940710795816,
flame,3.0,1913.55,0,0.4862702494211093,0.4218878452433271,0.6442579511796879,0.7037862995686953,0.39050816101559743,0.4615695027134954,0.4837665868329622,202.7214129395292,0.799521740580789,0.4120656817418856,
flame,4.0,1211.45,0,0.5401951313617974,0.5423000184997735,0.8281373895516299,0.6713416323651232,0.4008278323502659,0.4296731714964762,0.5372775422796912,258.16406743385016,0.6955953710582403,0.4426011973843992,
flame,5.0,1022.72,0,0.5256495878511207,0.5889556160037883,0.8993843808975512,0.6050194209391393,0.3713407501938503,0.3477673085111003,0.5220412914409845,239.22155721975062,0.8354291986139307,0.40290334974973696,
insect,2.0,10683.5,0,0.5714653581432843,0.506210859163194,0.4607729809548126,0.6920827420915049,0.7521576281325172,0.4680581910183429,0.5532686294745759,60.270752590319965,0.5799482315693878,0.5487736943919346,
insect,3.0,6002.75,1,0.6449126680040378,0.7053771852381958,0.6420619835714308,0.7399714201441608,0.647788778776089,0.6210196944597828,0.6188196252675324,62.24513348048811,0.6953071628687417,0.4687681249232857,
insect,4.0,4236.08,0,0.608739437554484,0.7529275783523527,0.6853442166254631,0.6024640760767093,0.5475380311755307,0.4506480558325025,0.567532700638249,60.239615997481955,0.7966716127699024,0.4367901247098583,
insect,5.0,3075.25,0,0.6225083430893742,0.8194198139949896,0.7458680577735064,0.6125306510286749,0.5341627402160611,0.4690392923266817,0.5691211202622894,62.19958404465761,0.6300622543768848,0.4946298994716379,
lsun,2.0,670.265,0,0.6491389545399219,0.5611197584224346,0.5396831285472399,0.8181307280119151,0.8142889578784085,0.6660385013251185,0.6481154029375052,385.69283212595434,0.9362326608721658,0.4606180392796291,
lsun,3.0,381.64599999999996,1,0.5400568656616177,0.5655071130232259,0.5439028716973618,0.6423892311282245,0.5362648689101579,0.4358084271876845,0.5378309512789192,487.9512441770458,0.761378721589555,0.4967022054099482,
lsun,4.0,202.50400000000002,0,0.7222378729708145,0.8648766312254383,0.8318354845664621,0.7254440500031895,0.6381580310742303,0.5868596025789136,0.7204692059389957,728.3004198673977,0.5579387214345408,0.5655319907213792,
lsun,5.0,143.899,0,0.8040765861704536,1.039720770839918,1.0000000000000002,0.7712101533765884,0.6723478919069458,0.6477916751094491,0.8025284399220705,806.9620443446847,0.5826937708312114,0.5666015023842174,
pathbased,2.0,13638.3,0,0.4909971532293818,0.4392356920521657,0.4007586114577128,0.6519055872239359,0.6336831547050913,0.3989713297894657,0.4890804951430663,371.05530300508264,0.7522586238450906,0.5150123044043785,
pathbased,3.0,8957.91,1,0.5458430500422186,0.5620602381069193,0.512823717778765,0.6616839023616249,0.5834070523255318,0.4613289348654504,0.5428393181773931,359.10473171402344,0.6692535513389878,0.5419218557223351,
pathbased,4.0,7230.33,0,0.4658578423230228,0.5496313607454874,0.5014836110354494,0.580607790951345,0.4349580956992333,0.3827734541613793,0.4612180471591814,319.18113373464166,0.8696701159591098,0.4352170786214091,
pathbased,5.0,5901.86,0,0.4666431283706784,0.5981987867410505,0.545796526757575,0.5838176774556085,0.4075401699442199,0.4076167756503256,0.460928129070025,308.8800396373083,0.9428932950905058,0.3825725727537546,


==> Exact clustering with SOS-SDPA_arxiv/artificial_data_summary_clust_eval_tab.tex <==
\pgfplotstableread[col sep=comma]{artificial_data_summary_all_label_clust_eval.tex}\data
	\pgfplotstabletypeset[
	font=\footnotesize,
	multicolumn names, % allows to have multicolumn names
	columns={dataname,k, opt_sos_sdp,adjusted_mutual_info_score,adjusted_rand_score,homogeneity_score,completeness_score,normalized_mutual_info_score,fowlkes_mallows_score,calinski_harabasz_score,davies_bouldin_score,silhouette_score},
	fixed zerofill,
	fixed,
 	columns/dataname/.style={string type,
		column name={instances}
	},
	columns/k/.style={int detect,
		column name={$k$},
	},  
   columns/opt_sos_sdp/.style={precision=0,
        column name = {$d_{SOS}$},
        assign column name/.style={/pgfplots/table/column name={\multicolumn{1}{c|}{##1}}}
    },
	columns/homogeneity_score/.style={precision=2,
	column name={$h$},	},
	columns/completeness_score/.style={precision=2,column name={$c$},
	},
	columns/normalized_mutual_info_score/.style={precision=2,
	column name={NMI},
	},
	columns/fowlkes_mallows_score/.style={precision=2,
	column name={FMS},
	 assign column name/.style={
		/pgfplots/table/column name={\multicolumn{1}{c|}{##1}}}
	},
	columns/adjusted_mutual_info_score/.style={precision=2,column name={AMI},
	},
	columns/adjusted_rand_score/.style={precision=2,column name={ARS},
	},
	columns/calinski_harabasz_score/.style={precision=2,column name={CHC},
	},
	columns/davies_bouldin_score/.style={precision=2,column name={DBI},
	},
	columns/silhouette_score/.style={precision=2,column name={$S_{score}$},
	},
	row AMIS/.style={
	every row #1 column 3/.style={
	% postproc cell content/.append style={
	    % /pgfplots/table/@cell content/.add={\cellcolor{red!10!white}}{}}
    postproc cell content/.style={
          @cell content/.add={$\bf}{$}}	
 }
	},
	row ARS/.style={
	every row #1 column 4/.style={
	% postproc cell content/.append style={
	    % /pgfplots/table/@cell content/.add={\cellcolor{red!10!white}}{}}
    postproc cell content/.style={
          @cell content/.add={$\bf}{$}}	
 }
	},
	row c/.style={
	every row #1 column 5/.style={
	% postproc cell content/.append style={
	    % /pgfplots/table/@cell content/.add={\cellcolor{red!10!white}}{}}
    postproc cell content/.style={
          @cell content/.add={$\bf}{$}}	
 }
	},
	row h/.style={
	every row #1 column 6/.style={
	% postproc cell content/.append style={
	    % /pgfplots/table/@cell content/.add={\cellcolor{red!10!white}}{}}
     postproc cell content/.style={
          @cell content/.add={$\bf}{$}}
	}
	},
	row NMIS/.style={
	every row #1 column 7/.style={
	% postproc cell content/.append style={
	    % /pgfplots/table/@cell content/.add={\cellcolor{red!10!white}}{}}
	postproc cell content/.style={
          @cell content/.add={$\bf}{$}}
    }
	},
	row FMS/.style={
	every row #1 column 8/.style={
	% postproc cell content/.append style={
	    % /pgfplots/table/@cell content/.add={\cellcolor{red!10!white}}{}}
    postproc cell content/.style={
          @cell content/.add={$\bf}{$}}	
 }
	},
	row CHC/.style={
	every row #1 column 9/.style={
	  % postproc cell content/.append style={
            % /pgfplots/table/@cell content/.add={\cellcolor{red!10!white}}{} }
	 postproc cell content/.style={
          @cell content/.add={$\bf}{$}}   
     }
	},
	row DBI/.style={
	every row #1 column 10/.style={
	  % postproc cell content/.append style={
            % /pgfplots/table/@cell content/.add={\cellcolor{red!10!white}}{} }
            postproc cell content/.style={
          @cell content/.add={$\bf}{$}}
	    }
	},
	row s/.style={
	every row #1 column 11/.style={
	  % postproc cell content/.append style={
            % /pgfplots/table/@cell content/.add={\cellcolor{red!10!white}}{} 
    postproc cell content/.style={
          @cell content/.add={$\bf}{$}}
            % }
	    }
	},
    row AMIS/.list={1,7,12,18,20,26,31,36,41,46,51,56},
	row ARS/.list={4,7,12,16,20,25,29,33,39,46,51,56},
	row c/.list={4,7,12,18,20,24,29,36,38,46,48,53},
	row h/.list={4,9,12,18,20,27,31,36,41,46,51,56},
	row NMIS/.list={4,7,12,18,20,25,31,36,39,46,51,56,},
	row FMS/.list={4,7,12,16,20,25,29,33,39,46,51,56},
	row CHC/.list={4,9,12,18,20,25,31,36,38,46,51,55},
	row DBI/.list={3,9,12,18,20,24,30,35,39,46,50,54},
	row s/.list={2,6,12,18,20,24,29,36,39,46,51,55},
	rows truelabel/.style={
    every row no #1/.style={
    before row={\rowcolor[gray]{0.9}}},
    % postproc cell content/.style={
          % @cell content/.add={$\bf}{$}},
    },
    rows truelabel/.list={0,5,10,15,19,23,28,32,37,42,47,52},
	columns addvline/.style={
	every col no #1/.style={
	column type/.add={}{|}}
    },
    column type=r,
	columns addvline/.list={2,8},
	every head row/.style={
	before row={
	\caption{Clustering evaluations for artificial data} \label{tab:artificial_data_eval_clust} \\
	\toprule
	&  & &  \multicolumn{6}{c|}{extrinsic measurements}& \multicolumn{3}{c}{intrinsic measurements}\\
	},
	after row={
% 	&  &  &  & (rounded) &  (\si{\second}) & (rounded) & (\si{\second}) & \% &  &  &  
	\endfirsthead
	\midrule}
	},
	every last row/.style={after row=\bottomrule}
	]{\data} % filename/path to file
	
	

==> Exact clustering with SOS-SDPA_arxiv/artificial_data_summary_tab.tex <==
\pgfplotstableread[col sep=comma]{artificial_data_summary.tex}\data
	\pgfplotstabletypeset[
	font=\footnotesize,
	multicolumn names, % allows to have multicolumn names
	columns={name,type,n,m,K,M},
	fixed zerofill,
	fixed,
 	columns/name/.style={string type,
		column name={instances}
	},
	columns/type/.style={string type,
		column name={type}
	},
	columns/m/.style={int detect,
		column name={$m$},
	},
    columns/n/.style={int detect,
		column name={$n$},
	},
	columns/K/.style={int detect,
		column name={$k_{true}$},
	},
        columns/M/.style={string type,
		column name={measuring type},
	},  
	column type=r,
	every head row/.style={
	before row={
	\caption{Summarized information for artificial data} \label{tab:artificial_data_sum} \\
	\toprule
% 	&  &  \multicolumn{6}{c|}{extrinsic measurements}& \multicolumn{3}{c}{intrinsic measurements}\\
	},
	after row={
% 	&  &  &  & (rounded) &  (\si{\second}) & (rounded) & (\si{\second}) & \% &  &  &  
	\endfirsthead
	\midrule}
	},
	every last row/.style={after row=\bottomrule}
	]{\data} % filename/path to file
	
	

==> Exact clustering with SOS-SDPA_arxiv/real_data_summary.tex <==
name,type,n,m,K, M
dermatology,real,358,35,6, mixed
ecoli,real,336,8,8,numerical
glass,real,214,10,7, numerical
haberman,real,306,4,2, numerical
heart-statlog,real,270,14,2, mixed
iono,real,351,35,2, numerical
iris,real,150,5,3, numerical
sonar,real,208,61,2, numerical
tae,real,151,6,3, mixed
thy,real,215,6,3, numerical 
wine,real,178,14,3, numerical
%wisc,real,699,10,2
zoo,real,101,17,7, categorical


==> Exact clustering with SOS-SDPA_arxiv/real_data_summary_all_label_clust_eval.tex <==
dataname,k,opt_sos_sdp,normalized_mutual_info_score,mutual_info_score,homogeneity_score,fowlkes_mallows_score,completeness_score,adjusted_rand_score,adjusted_mutual_info_score,calinski_harabasz_score,davies_bouldin_score,silhouette_score
arrhythmia,3.0,16621623.2990983,1.0,1.664514143432401,1.0,1.0,1.0,1.0,1.0,7.3538326473514335,3.99676672946264,-0.0250518944110154
arrhythmia,2.0,17873000.0,0.0311133712137884,0.0363669388011164,0.0218483807690116,0.4239995598434332,0.0540217511950851,0.023554266039522,0.0187408106998119,52.61608034768564,2.654391799943445,0.1261106391687146
arrhythmia,3.0,16838500.0,0.1296017009246813,0.1666980831688465,0.1001481926882866,0.4287654161535796,0.1835976243131432,0.0817991547272355,0.1096691986306355,41.65533164260298,2.532531179757959,0.0976110690661389
arrhythmia,4.0,15929100.0,0.1602572886316708,0.2201493289433538,0.1322604135338754,0.4378424830046956,0.2032896215126699,0.1273054528652708,0.1336420160051497,37.81602509175721,2.3000398622870994,0.0951958714299945
arrhythmia,5.0,15241000.0,0.1625611349497498,0.2523178570154988,0.1515864902746895,0.3644819235477951,0.1752489045074288,0.1053165712552402,0.1305508149498917,34.62150334727939,2.4259279061575683,0.0763140260241946
arrhythmia,6.0,14588400.0,0.1702231406769618,0.2660839897923807,0.1598568512272823,0.3667281236518344,0.1820271122876649,0.1098105634875947,0.1356665090835094,32.861907093261394,2.1046638720575146,0.0785622856050936
arrhythmia,7.0,13955400.0,0.1896998322294754,0.3008503889776913,0.1807436663513754,0.3653351146137732,0.1995898600825743,0.1100530620563422,0.151059984856815,31.926916875762117,1.9796163874290629,0.0893736745008537
balance-scale,3.0,,1.0,0.91364855987124,1.0,1.0,1.0,1.0,1.0,63.395442099716654,4.218747293065079,0.0888307913921624
balance-scale,2.0,4062.5,0.0533186532336323,0.0428352393431122,0.046883715713566,0.5041814760723365,0.061801040527784,0.0758211964357062,0.0514170465731192,143.76923076923077,2.01857949405675,0.1819410926722415
dermatology,6.0,71575.45485344502,1.0,1.6832739364924156,1.0,1.0,1.0,1.0,1.0,20.679657647590588,5.89901002547441,-0.0335783541649112
dermatology,4.0,16162.4,0.0837777622186428,0.1269530274813306,0.0754203013122592,0.2526072253328422,0.0942182590471259,0.0276453102830479,0.070566805693841,558.0661308282387,0.8923486314414688,0.3489327873326072
dermatology,5.0,13364.9,0.1095777420570606,0.1766180225193485,0.1049252998518963,0.2394009308147556,0.1146619106332565,0.0354501534209339,0.0932367382420944,523.1991232483508,0.9420232132816876,0.3192755968323302
dermatology,6.0,11698.0,0.1077224207166259,0.183017909029585,0.1087273467864389,0.2157509523425433,0.1067359008345187,0.0265942727992582,0.0880755985488046,486.8794773046705,1.0589993360439955,0.2864864243102078
dermatology,7.0,10552.3,0.1048528806488991,0.1879476552808499,0.1116560122546023,0.1979203758764419,0.0988311593782073,0.0281374558429034,0.0822901312897753,454.8607809904705,1.207820098125675,0.2598450604236552
dermatology,8.0,9831.41,0.1772437187904006,0.3290176844917573,0.195462947152476,0.2181678945846156,0.1621313502430022,0.0630829923519399,0.1536292513311843,420.94172423979455,1.2225216095179965,0.2613383722102094
ecoli,8.0,21.306504120879126,1.0,1.517122829952031,1.0,1.0,1.0,1.0,1.0,81.17586758649125,1.5753319355303452,0.2382407258501354
ecoli,6.0,16.5347,0.621433531799543,0.9901249222167764,0.652633328474849,0.6165667143315855,0.5930807083894373,0.4936599210527242,0.6083844151951374,166.38453535988808,1.264422122110093,0.2809992948229829
ecoli,7.0,15.0043,0.6237586989449899,1.0293283922625398,0.6784739982425059,0.6418754378490984,0.5772098144799364,0.5265993900048032,0.6089821609647691,157.92598780623803,1.229209297964023,0.2734487842081349
ecoli,8.0,13.848,0.6162561974225754,1.0753129421737673,0.708784365342236,0.5605420133404836,0.54509662540823,0.426192978871245,0.5996568042730128,150.13386710651346,1.2212185354020693,0.2540869241157364
ecoli,9.0,12.9786,0.6504800716742517,1.1524170933524711,0.7596069814524568,0.5758129991080211,0.5687693420588131,0.4435754287012778,0.6338409588866849,142.47844313205275,1.1624952775469637,0.2649987522623291
ecoli,10.0,12.2649,0.6557502472519027,1.16832132641489,0.770090135979188,0.576594900482865,0.5709742805737514,0.4444173551129747,0.6380161381587897,135.71435262960037,1.1207675015930014,0.270912320776119
glass,6.0,911.2040712197261,1.0,1.5086584002236936,1.0,1.0,1.0,1.0,1.0,19.702067127104986,3.73631979010432,-0.0914413867182059
glass,5.0,400.259,0.3772224403230368,0.5043250206736848,0.3342870861945334,0.4978578683426982,0.4328122216009364,0.2520460591021136,0.3532086463841432,123.03415777775744,0.9042043494669332,0.4426886725031028
glass,6.0,336.061,0.4157375276959366,0.5707364427990196,0.3783072713573826,0.4986501147071163,0.4613878987846299,0.255213359620384,0.3879403868556083,124.61616247195136,0.9350845435798436,0.4468862914963273
glass,7.0,292.254,0.4242314831428778,0.6024588284534091,0.3993341556737301,0.4976789511947704,0.4524397932313275,0.267756636335495,0.3928546495972367,124.00967694153962,0.8741233438503606,0.4550617511042344
glass,8.0,266.496,0.4539089159703398,0.6571087899089563,0.4355583674949376,0.5073453178437526,0.4738737325107051,0.2792875315533171,0.4197452779369728,118.84939171483424,0.8579717871319198,0.4574789512940245
glass,9.0,245.351,0.4084028991390969,0.6664680570982393,0.4417620695310615,0.4075664886202422,0.3797281509776367,0.2224588792384759,0.3706311820149561,114.61555420318405,0.9710525084978392,0.3041441401748521
haberman,2.0,53123.17333333333,1.0,0.5779217946828967,1.0,1.0,1.0,1.0,1.0,8.360345155772595,4.725836847244438,0.0597219507631459
haberman,2.0,30507.0,7.965736046142885e-05,5.050237119169632e-05,8.7386168260719e-05,0.5519976954266277,7.318460028939525e-05,-0.0018130326610555,-0.0025219560050244,239.92636004273905,0.9687879726138507,0.4012977121920988
haberman,3.0,21164.6,0.0361368231690338,0.0274498400271737,0.0474974992805649,0.5319055614762077,0.0291617727025833,0.0522418524106729,0.0319025371591291,239.22305793227412,0.8473812792396576,0.4316143935765462
haberman,4.0,15366.5,0.0225034689759232,0.0210744260091325,0.0364658786068034,0.4365966353327911,0.0162727864971384,0.0273170705144174,0.0172778467931294,256.9162536550288,0.8533987498306269,0.3719096040767244
heart-statlog,2.0,934653.3878499997,1.0,0.6869615765973238,1.0,1.0,1.0,1.0,1.0,11.137445285462835,4.156427207730943,0.0501465917975156
heart-statlog,2.0,549315.0,0.0199122924571302,0.0134400738960099,0.0195645205698136,0.5307324925591533,0.0202726518312902,0.0302303325860961,0.017199186261725,206.9495407269051,0.9871370082638804,0.3804182800071519
heart-statlog,3.0,431736.0,0.0139079599739712,0.0121248819526923,0.0176500147399067,0.4312904396637974,0.0114750795137229,0.0106123234232289,0.0096650455661279,167.52135434182202,1.1633560674055936,0.2773423952865388
heart-statlog,4.0,351403.0,0.025088024444836,0.0231136120846906,0.0336461497587355,0.4213882389610534,0.0200007090790926,0.0228636819864862,0.0188163950819586,156.96769726829186,1.0773743172759558,0.2754035733026458
iono,2.0,3086.176177564397,1.0,0.6528257939163475,1.0,1.0,1.0,1.0,1.0,17.74606012127195,4.08644491721087,0.1548790250623376
iono,2.0,2419.36,0.13485692093441,0.0905264814101238,0.1386686651381361,0.6052850553774272,0.1312491260868341,0.177606854737686,0.1330081904044343,118.82649338303231,1.513475950743014,0.2959701497777325
iono,3.0,2193.32,0.192828707888386,0.1569871352216589,0.240473242149153,0.587003830812214,0.1609416299929337,0.2200462194832898,0.1899676707646518,83.28120876024403,1.8019594860993509,0.2884590817381463
iono,4.0,1999.18,0.2380034420870625,0.2194422392554498,0.3361421091207204,0.5775331551770819,0.1842194805618035,0.2437927008085461,0.2344108128480203,71.96981929435267,1.7104687629047608,0.3057357408709429
iris,3.0,89.38680000000001,1.0,1.0986122886681096,1.0,1.0,1.0,1.0,1.0,486.3208393185568,0.7517428073901344,0.5032506980366628
iris,2.0,152.369,0.6565191143081124,0.5738298777087831,0.5223224641010155,0.7504732564880243,0.8835142349190769,0.5399218294207123,0.6538380713762781,513.3038433517569,0.4048341363918284,0.680813620271351
iris,3.0,78.9408,0.7581756800057784,0.8255910976103356,0.7514854021988338,0.8208080729114153,0.7649861514489815,0.7302382722834697,0.7551191675800485,560.3999242466399,0.6623228649898628,0.552591944521368
iris,4.0,57.3179,0.7219203867820961,0.8880235203213085,0.8083138423637095,0.7565926353252695,0.6522113355514313,0.6498176853819967,0.7172081944051022,529.3982941434153,0.780640036237599,0.4978256900754499
iris,5.0,46.5356,0.6938628345588717,0.9051279136224294,0.8238829320940431,0.7254830776265845,0.59928706467119,0.6078964652364223,0.6872109247445372,494.0943819140987,0.80624149219652,0.4885175508538638
sonar,2.0,351.5856632023387,1.0,0.690880304410466,1.0,1.0,1.0,1.0,1.0,6.004452460055308,5.685775044966328,0.0301424569014513
sonar,2.0,280.534,0.0087901130807924,0.0060755607287341,0.0087939411356045,0.5027663757107326,0.0087862883572801,0.0064098447858296,0.0053052470002705,59.699458265423424,1.8005189338588006,0.1983999469666345
sonar,3.0,235.04,0.0031105584580843,0.0027476044649865,0.0039769616349551,0.4143222590518839,0.0025541275810736,-0.0017586922582194,-0.0024019487046078,55.29428177572339,1.6929144859460152,0.1924868838776389
sonar,4.0,217.165,0.0232080086074249,0.0233604906702342,0.0338126452890678,0.3853278410759623,0.0176670910080888,0.0205020854733452,0.0160545336776992,45.29926475510734,1.907214357311025,0.173614025494858
tae,3.0,38345.79758241758,1.0,1.0983062060529227,1.0,1.0,1.0,1.0,1.0,1.975107479601828,9.1301455401467,-0.0191986930578776
tae,2.0,21803.3,0.0070823307737267,0.0062585814620781,0.0056983939702664,0.414028536176009,0.0093541109382047,0.0001139684162335,-0.0005244138766196,120.04262044283244,1.0472127358490746,0.3801283934670079
tae,3.0,16775.4,0.0263141921557827,0.027684818359896,0.0252068304880015,0.3619355927406001,0.0275233195406774,0.0088791124595939,0.013589272548773,99.66676208871986,1.1042788462657311,0.3374766558094673
tae,4.0,13221.3,0.0381660879455284,0.0460054335294892,0.041887620479559,0.3111809990024711,0.0350518810681581,0.0079944491521073,0.0215936711539228,96.90851752548882,1.103668339637843,0.3432389497757682
tae,5.0,10537.7,0.0461049400266953,0.0612875787555209,0.0558019051679362,0.2779161092756532,0.0392792040381583,0.0141953136972677,0.0260880765325214,99.86594938807347,0.9866865681764873,0.3643123596056096
thy,3.0,38859.19328571429,1.0,0.8214826899116975,1.0,1.0,1.0,1.0,1.0,68.80148036158958,1.2444333530707423,0.3835002853016623
thy,2.0,41608.0,0.1276326688305902,0.0966408677875019,0.1176420014375349,0.5372099535501407,0.1394777198380171,0.0477515733517705,0.1221508130975099,115.04657594115812,1.0656984721770733,0.3462207447643413
thy,3.0,28560.2,0.4945160467056619,0.3986646698203863,0.4852989292607485,0.8062522135438603,0.5040900576587282,0.5790671581240897,0.4882857152795125,131.83643925618364,0.923577781311556,0.4565740832904507
thy,4.0,20082.7,0.3211378902629165,0.3032556869761809,0.3691565150432791,0.6175825442367808,0.2841735594981179,0.2814179070237005,0.3100305802062995,154.09183040925103,0.8249080653270505,0.4107051556699644
thy,5.0,15402.5,0.3311263808530725,0.3542028607238399,0.4311750753529739,0.5803410290976675,0.2687632789007592,0.275402190922566,0.318149238984441,165.92420027947998,0.8300573416438153,0.3944580789974784
wine,3.0,33788.03886609779,1.0,1.0860384436406825,1.0,1.0,1.0,1.0,1.0,15.81175326135954,2.806900926429026,0.0688642280213505
wine,2.0,4543750.0,0.4259186266746114,0.3629524368591491,0.3341985166219701,0.6590510206234098,0.587027006858955,0.3694075388574537,0.4220526675739516,19.490035043004056,2.176493391527308,0.1139838328809922
wine,3.0,2370690.0,0.4287568597645354,0.4657066646034707,0.4288123199785646,0.5835370218944976,0.4287014138944858,0.3711137182308475,0.4226866642766121,18.638514675777287,4.303568871252648,0.040614246164066
wine,4.0,1331900.0,0.3884332923957888,0.4644628506130969,0.4276670437706578,0.5207343245323419,0.3557931783115363,0.303442531578347,0.3794660493529976,11.956480798763463,7.735705077833749,-0.0318784506667515
wine,5.0,916379.0,0.4109925606542485,0.537739887874978,0.4951389069362355,0.5087079622475457,0.351292227983938,0.3115880103317625,0.4003850916370255,14.735786788755284,5.408027216584347,-0.058420718797689
zoo,7.0,277.96510318949345,1.0,1.657009703742392,1.0,1.0,1.0,1.0,1.0,23.902799308963928,1.8586399351741556,0.3039716264714694
zoo,5.0,158.63,0.6993349994752281,1.0984475727336185,0.6629095594628994,0.680681732167751,0.7399961819075096,0.5811563562389545,0.6707532901380499,82.21871061168216,0.9255466297226396,0.4301899320142995
zoo,6.0,134.773,0.745044183859346,1.235315542067745,0.7455089365365565,0.7363517316948206,0.7445800102777634,0.6610838742714487,0.7159708514353341,79.97448856682449,0.9310474847925786,0.4477971563030443
zoo,7.0,119.704,0.7816625894813721,1.3471139658020228,0.8129789238768711,0.7741355207962075,0.7526694063540147,0.7087529337715824,0.7527195513185745,76.21779577510424,1.0211302587108235,0.4405712903716863
zoo,8.0,109.287,0.8078200013977627,1.4227394115400198,0.8586186359239372,0.787945046988338,0.7626964323306963,0.7251155013659698,0.7790454380030649,72.06147916786657,1.0561214365381415,0.442117718340804
zoo,9.0,100.129,0.8337886459103071,1.5011749300384132,0.90595421779847,0.8072445195129591,0.7722718101398626,0.74711213630809,0.8062558551394664,69.13282029937969,0.9903091219416648,0.4547490257242741


==> Exact clustering with SOS-SDPA_arxiv/real_data_summary_clust_eval.tex <==
dataname,k,opt_sos_sdp,true_k,normalized_mutual_info_score,mutual_info_score,homogeneity_score,fowlkes_mallows_score,completeness_score,adjusted_rand_score,adjusted_mutual_info_score,calinski_harabasz_score,davies_bouldin_score,silhouette_score,
arrhythmia,2.0,17873000.0,0,0.03111337121378848,0.03636693880111641,0.02184838076901168,0.4239995598434333,0.054021751195085135,0.023554266039522005,0.01874081069981196,52.616080347685646,2.6543917999434483,0.12611063916871462,
arrhythmia,3.0,16838500.0,0,0.1296017009246813,0.1666980831688465,0.10014819268828663,0.4287654161535796,0.18359762431314328,0.08179915472723552,0.10966919863063558,41.65533164260298,2.5325311797579544,0.09761106906613894,
arrhythmia,4.0,15929100.0,0,0.16025728863167088,0.22014932894335384,0.13226041353387544,0.4378424830046957,0.20328962151267,0.12730545286527087,0.13364201600514974,37.81602509175721,2.300039862287101,0.0951958714299946,
arrhythmia,5.0,15241000.0,0,0.16256113494974986,0.2523178570154988,0.1515864902746895,0.3644819235477951,0.17524890450742886,0.10531657125524024,0.13055081494989176,34.62150334727939,2.425927906157564,0.0763140260241947,
arrhythmia,6.0,14588400.0,0,0.1702231406769618,0.2660839897923807,0.15985685122728238,0.3667281236518344,0.18202711228766494,0.10981056348759476,0.13566650908350944,32.861907093261394,2.1046638720575164,0.07856228560509364,
arrhythmia,7.0,13955400.0,0,0.18969983222947548,0.3008503889776913,0.18074366635137545,0.3653351146137732,0.19958986008257434,0.11005306205634223,0.15105998485681507,31.926916875762114,1.979616387429061,0.0893736745008538,
balance-scale,2.0,4062.5,0,0.053318653233632315,0.04283523934311223,0.04688371571356603,0.5041814760723365,0.061801040527784075,0.07582119643570624,0.05141704657311922,143.76923076923075,2.01857949405675,0.1819410926722415,
dermatology,4.0,16162.4,0,0.08377776221864286,0.12695302748133064,0.0754203013122592,0.2526072253328422,0.09421825904712597,0.02764531028304793,0.07056680569384108,558.0661308282387,0.8923486314414679,0.34893278733260724,
dermatology,5.0,13364.9,0,0.10957774205706064,0.17661802251934858,0.10492529985189633,0.2394009308147557,0.11466191063325652,0.03545015342093395,0.0932367382420944,523.1991232483508,0.9420232132816873,0.3192755968323302,
dermatology,6.0,11698.0,1,0.10772242071662592,0.18301790902958506,0.10872734678643893,0.21575095234254332,0.10673590083451877,0.02659427279925827,0.0880755985488046,486.8794773046705,1.0589993360439955,0.2864864243102078,
dermatology,7.0,10552.3,0,0.10485288064889917,0.18794765528084995,0.11165601225460238,0.19792037587644196,0.0988311593782073,0.02813745584290346,0.08229013128977533,454.8607809904705,1.207820098125675,0.25984506042365524,
dermatology,8.0,9831.41,0,0.17724371879040066,0.3290176844917573,0.195462947152476,0.21816789458461566,0.16213135024300224,0.06308299235193998,0.15362925133118432,420.94172423979455,1.2225216095179972,0.2613383722102094,
ecoli,6.0,16.5347,0,0.621433531799543,0.9901249222167764,0.652633328474849,0.6165667143315855,0.5930807083894373,0.4936599210527242,0.6083844151951374,166.3845353598881,1.2644221221100922,0.280999294822983,
ecoli,7.0,15.0043,0,0.6237586989449899,1.0293283922625398,0.6784739982425059,0.6418754378490984,0.5772098144799364,0.5265993900048032,0.6089821609647691,157.92598780623803,1.2292092979640221,0.2734487842081351,
ecoli,8.0,13.847999999999999,1,0.6162561974225754,1.0753129421737673,0.708784365342236,0.5605420133404836,0.54509662540823,0.426192978871245,0.5996568042730128,150.13386710651346,1.2212185354020686,0.2540869241157365,
ecoli,9.0,12.9786,0,0.6504800716742517,1.1524170933524711,0.7596069814524568,0.5758129991080211,0.5687693420588131,0.4435754287012778,0.6338409588866849,142.47844313205275,1.162495277546962,0.2649987522623294,
ecoli,10.0,12.2649,0,0.6557502472519027,1.16832132641489,0.770090135979188,0.576594900482865,0.5709742805737514,0.4444173551129748,0.6380161381587897,135.71435262960034,1.1207675015930003,0.2709123207761192,
glass,5.0,400.259,0,0.3772224403230369,0.5043250206736848,0.33428708619453346,0.4978578683426982,0.4328122216009364,0.25204605910211364,0.3532086463841432,123.03415777775743,0.9042043494669558,0.44268867250311705,
glass,6.0,336.061,1,0.41573752769593664,0.5707364427990196,0.3783072713573826,0.4986501147071163,0.4613878987846299,0.25521335962038405,0.3879403868556083,124.61616247195136,0.9350845435798348,0.44688629149634107,
glass,7.0,292.254,0,0.42423148314287773,0.6024588284534091,0.39933415567373015,0.4976789511947705,0.4524397932313275,0.267756636335495,0.3928546495972368,124.00967694153962,0.8741233438503809,0.4550617511042501,
glass,8.0,266.496,0,0.4539089159703398,0.6571087899089563,0.4355583674949377,0.5073453178437526,0.4738737325107051,0.27928753155331715,0.4197452779369728,118.84939171483423,0.8579717871319328,0.4574789512940386,
glass,9.0,245.351,0,0.4084028991390969,0.6664680570982393,0.4417620695310615,0.4075664886202423,0.3797281509776368,0.2224588792384759,0.37063118201495615,114.61555420318405,0.9710525084978312,0.30414414017487085,
haberman,2.0,30507.0,1,7.965736046142884e-05,5.050237119169632e-05,8.738616826071899e-05,0.5519976954266277,7.318460028939525e-05,-0.001813032661055529,-0.0025219560050244805,239.92636004273902,0.9687879726138507,0.4012977121920989,
haberman,3.0,21164.6,0,0.03613682316903384,0.02744984002717371,0.04749749928056498,0.5319055614762077,0.0291617727025833,0.052241852410672925,0.03190253715912912,239.22305793227414,0.8473812792396576,0.4316143935765462,
haberman,4.0,15366.5,0,0.022503468975923268,0.021074426009132518,0.03646587860680349,0.4365966353327911,0.01627278649713847,0.02731707051441749,0.01727784679312943,256.9162536550288,0.8533987498306269,0.3719096040767245,
heart-statlog,2.0,549315.0,1,0.019912292457130217,0.013440073896009984,0.01956452056981369,0.5307324925591533,0.020272651831290223,0.030230332586096142,0.017199186261725025,206.9495407269051,0.9871370082638804,0.3804182800071519,
heart-statlog,3.0,431736.0,0,0.013907959973971276,0.012124881952692318,0.01765001473990671,0.43129043966379743,0.0114750795137229,0.010612323423228943,0.009665045566127932,167.52135434182205,1.163356067405595,0.2773423952865388,
heart-statlog,4.0,351403.0,0,0.02508802444483609,0.023113612084690628,0.03364614975873553,0.42138823896105343,0.020000709079092627,0.022863681986486247,0.018816395081958613,156.9676972682919,1.0773743172759576,0.2754035733026457,
iono,2.0,2419.36,1,0.13485692093441007,0.09052648141012387,0.13866866513813614,0.6052850553774272,0.13124912608683412,0.17760685473768606,0.13300819040443435,118.82649338303233,1.5134759507430142,0.2959701497777326,
iono,3.0,2193.32,0,0.19282870788838605,0.1569871352216589,0.24047324214915305,0.587003830812214,0.16094162999293374,0.22004621948328987,0.18996767076465187,83.28120876024404,1.8019594860993509,0.2884590817381463,
iono,4.0,1999.18,0,0.23800344208706256,0.2194422392554498,0.3361421091207204,0.5775331551770819,0.1842194805618036,0.2437927008085461,0.2344108128480203,71.96981929435267,1.7104687629047608,0.3057357408709429,
iris,2.0,152.369,0,0.6565191143081124,0.5738298777087831,0.5223224641010155,0.7504732564880243,0.8835142349190769,0.5399218294207123,0.6538380713762781,513.3038433517569,0.40483413639182864,0.6808136202713507,
iris,3.0,78.9408,1,0.7581756800057784,0.8255910976103356,0.7514854021988338,0.8208080729114153,0.7649861514489815,0.7302382722834697,0.7551191675800485,560.3999242466399,0.6623228649898673,0.5525919445213676,
iris,4.0,57.3179,0,0.7219203867820961,0.8880235203213085,0.8083138423637095,0.7565926353252695,0.6522113355514313,0.6498176853819967,0.7172081944051022,529.3982941434153,0.7806400362376116,0.4978256900754493,
iris,5.0,46.5356,0,0.6938628345588717,0.9051279136224294,0.8238829320940431,0.7254830776265845,0.59928706467119,0.6078964652364223,0.6872109247445372,494.0943819140987,0.8062414921965185,0.4885175508538632,
sonar,2.0,280.534,1,0.008790113080792413,0.006075560728734164,0.008793941135604513,0.5027663757107326,0.008786288357280174,0.006409844785829633,0.00530524700027054,59.699458265423424,1.8005189338587992,0.1983999469666345,
sonar,3.0,235.04,0,0.003110558458084321,0.002747604464986592,0.003976961634955198,0.414322259051884,0.0025541275810736863,-0.0017586922582194335,-0.0024019487046078613,55.29428177572339,1.6929144859460152,0.19248688387763896,
sonar,4.0,217.165,0,0.023208008607424925,0.02336049067023427,0.0338126452890678,0.3853278410759623,0.01766709100808889,0.020502085473345238,0.016054533677699222,45.299264755107345,1.9072143573110252,0.1736140254948581,
tae,2.0,21803.3,0,0.007082330773726759,0.0062585814620781674,0.005698393970266422,0.41402853617600893,0.009354110938204796,0.00011396841623356773,-0.0005244138766196055,120.04262044283243,1.0472127358490746,0.3801283934670079,
tae,3.0,16775.4,1,0.02631419215578276,0.02768481835989608,0.02520683048800151,0.36193559274060016,0.02752331954067745,0.00887911245959397,0.013589272548773004,99.66676208871986,1.1042788462657307,0.3374766558094673,
tae,4.0,13221.3,0,0.03816608794552848,0.046005433529489256,0.04188762047955909,0.3111809990024711,0.035051881068158125,0.007994449152107399,0.021593671153922883,96.90851752548882,1.103668339637843,0.34323894977576824,
tae,5.0,10537.7,0,0.04610494002669531,0.06128757875552099,0.0558019051679362,0.2779161092756532,0.039279204038158336,0.014195313697267726,0.02608807653252143,99.86594938807349,0.9866865681764868,0.3643123596056097,
thy,2.0,41608.0,0,0.12763266883059027,0.09664086778750196,0.11764200143753492,0.5372099535501407,0.13947771983801716,0.04775157335177057,0.12215081309750993,115.04657594115812,1.0656984721770706,0.3462207447643411,
thy,3.0,28560.2,1,0.494516046705662,0.3986646698203863,0.4852989292607485,0.8062522135438603,0.5040900576587282,0.5790671581240897,0.4882857152795125,131.83643925618364,0.9235777813115492,0.4565740832904506,
thy,4.0,20082.7,0,0.32113789026291656,0.3032556869761809,0.3691565150432791,0.6175825442367808,0.2841735594981179,0.28141790702370056,0.31003058020629953,154.09183040925103,0.8249080653270541,0.4107051556699643,
thy,5.0,15402.5,0,0.3311263808530725,0.3542028607238399,0.431175075352974,0.5803410290976675,0.26876327890075924,0.27540219092256607,0.31814923898444103,165.92420027947995,0.8300573416438102,0.3944580789974783,
wine,2.0,4543750.0,0,0.42591862667461133,0.3629524368591491,0.3341985166219701,0.6590510206234098,0.5870270068589549,0.3694075388574537,0.4220526675739517,19.490035043004056,2.176493391527314,0.11398383288099236,
wine,3.0,2370690.0,1,0.4287568597645354,0.4657066646034707,0.4288123199785647,0.5835370218944976,0.42870141389448585,0.3711137182308475,0.4226866642766121,18.63851467577729,4.303568871252974,0.04061424616406595,
wine,4.0,1331900.0,0,0.3884332923957888,0.4644628506130969,0.42766704377065773,0.5207343245323419,0.3557931783115363,0.303442531578347,0.3794660493529976,11.956480798763465,7.735705077835789,-0.0318784506667515,
wine,5.0,916379.0,0,0.4109925606542485,0.537739887874978,0.4951389069362355,0.5087079622475457,0.351292227983938,0.3115880103317625,0.4003850916370255,14.735786788755286,5.408027216583188,-0.058420718797688974,
zoo,5.0,158.63,0,0.6993349994752281,1.0984475727336185,0.6629095594628994,0.6806817321677511,0.7399961819075096,0.5811563562389545,0.6707532901380499,82.21871061168216,0.9255466297226398,0.4301899320142995,
zoo,6.0,134.773,0,0.7450441838593459,1.235315542067745,0.7455089365365565,0.7363517316948206,0.7445800102777634,0.6610838742714487,0.7159708514353341,79.97448856682449,0.9310474847925786,0.4477971563030443,
zoo,7.0,119.704,1,0.7816625894813721,1.3471139658020228,0.8129789238768711,0.7741355207962075,0.7526694063540147,0.7087529337715824,0.7527195513185745,76.21779577510424,1.0211302587108235,0.4405712903716864,
zoo,8.0,109.287,0,0.8078200013977627,1.4227394115400198,0.8586186359239372,0.7879450469883381,0.7626964323306963,0.7251155013659698,0.7790454380030649,72.06147916786657,1.0561214365381413,0.442117718340804,
zoo,9.0,100.12899999999999,0,0.8337886459103071,1.5011749300384132,0.90595421779847,0.8072445195129591,0.7722718101398626,0.7471121363080899,0.8062558551394664,69.13282029937969,0.9903091219416648,0.4547490257242741,


==> Exact clustering with SOS-SDPA_arxiv/real_data_summary_clust_eval_tab.tex <==
% \resizebox{\linewidth}{!}{	
\pgfplotstableread[col sep=comma]{real_data_summary_all_label_clust_eval.tex}\data
 \pgfplotstabletypeset[
	font=\footnotesize,
	multicolumn names, % allows to have multicolumn names
	columns={dataname,k,opt_sos_sdp,adjusted_mutual_info_score,adjusted_rand_score,homogeneity_score,completeness_score,normalized_mutual_info_score,fowlkes_mallows_score,calinski_harabasz_score,davies_bouldin_score,silhouette_score},
	fixed zerofill,
	fixed,
 	columns/dataname/.style={string type,
		column name={instances}
	},
	columns/k/.style={int detect,
		column name={$k$},
		% assign column name/.style={
		% /pgfplots/table/column name={\multicolumn{1}{c|}{##1}}}
	},  
    columns/opt_sos_sdp/.style={precision=0,
        column name ={$d_{SOS}$.},
        assign column name/.style={/pgfplots/table/column name={\multicolumn{1}{c|}{##1}}}
    },
	columns/completeness_score/.style={precision=2,column name={$c$},
	},
    columns/homogeneity_score/.style={precision=2,
	column name={$h$},	},
	columns/normalized_mutual_info_score/.style={precision=2,
	column name={NMI},
	},
	columns/fowlkes_mallows_score/.style={precision=2,
	column name={FMS},
	  assign column name/.style={
		/pgfplots/table/column name={\multicolumn{1}{c|}{##1}}}
	},
	columns/adjusted_mutual_info_score/.style={precision=2,column name={AMI},
	},
	columns/adjusted_rand_score/.style={precision=2,column name={ARS},
	},
	columns/calinski_harabasz_score/.style={precision=2,column name={CHC},
	},
	columns/davies_bouldin_score/.style={precision=2,column name={DBI},
	},
	columns/silhouette_score/.style={precision=2,column name={$S_{score}$},
	},
    row truelabel/.style={
    every row no #1/.style={
    before row={\rowcolor[gray]{0.9}}},
    },
	% highlight best scores for each measurements
	row AMIS/.style={
	every row #1 column 3/.style={
	% postproc cell content/.append style={
	    % /pgfplots/table/@cell content/.add={\cellcolor{red!10!white}}{}}
     postproc cell content/.style={
          @cell content/.add={$\bf}{$}}
	}
	},
	row ARS/.style={
	every row #1 column 4/.style={
	% postproc cell content/.append style={
	    % /pgfplots/table/@cell content/.add={\cellcolor{red!10!white}}{}}
    postproc cell content/.style={
          @cell content/.add={$\bf}{$}}	
 }
	},
	row h/.style={
	every row #1 column 5/.style={
	% postproc cell content/.append style={
	    % /pgfplots/table/@cell content/.add={\cellcolor{red!10!white}}{}}
	postproc cell content/.style={
          @cell content/.add={$\bf}{$}}
    }
	},
	row c/.style={
	every row #1 column 6/.style={
	% postproc cell content/.append style={
	    % /pgfplots/table/@cell content/.add={\cellcolor{red!10!white}}{}}
    postproc cell content/.style={
          @cell content/.add={$\bf}{$}}	
 }
	},
	row NMIS/.style={
	every row #1 column 7/.style={
	% postproc cell content/.append style={
	    % /pgfplots/table/@cell content/.add={\cellcolor{red!10!white}}{}}
    postproc cell content/.style={
          @cell content/.add={$\bf}{$}}	
 }
	},
	row FMS/.style={
	every row #1 column 8/.style={
	% postproc cell content/.append style={
	    % /pgfplots/table/@cell content/.add={\cellcolor{red!10!white}}{}}
    postproc cell content/.style={
          @cell content/.add={$\bf}{$}}	
    }
	},
	row CHC/.style={
	every row #1 column 9/.style={
	  % postproc cell content/.append style={
            % /pgfplots/table/@cell content/.add={\cellcolor{red!10!white}}{} }
	 postproc cell content/.style={
          @cell content/.add={$\bf}{$}}   
     }
	},
	row DBI/.style={
	every row #1 column 10/.style={
	  % postproc cell content/.append style={
            % /pgfplots/table/@cell content/.add={\cellcolor{red!10!white}}{} }
	 postproc cell content/.style={
          @cell content/.add={$\bf}{$}}   
     }
	},
	row s/.style={
	every row #1 column 11/.style={
	  % postproc cell content/.append style={
            % /pgfplots/table/@cell content/.add={\cellcolor{red!10!white}}{} }
	 postproc cell content/.style={
          @cell content/.add={$\bf}{$}}   
     }
	},
	skip rows between index={0}{9},
	skip rows between index={26}{27},
	row truelabel/.list={0,6,12,17,21,25,29,34,38,43,48,53},
	row AMIS/.list={14,20,25,29,34,38,41,47,52,55,60,68},
	row ARS/.list={14,16,25,29,32,38,41,47,52,55,60,68},
	row h/.list={14,20,25,29,34,38,43,47,52,55,62,68},
	row c/.list={14,16,25,29,32,38,40,47,52,55,59,68},
	row NMIS/.list={14,20,25,29,34,38,41,47,52,55,60,68},
	row FMS/.list={10,17,25,28,32,36,41,45,49,55,59,,68},
	row CHC/.list={10,16,23,30,32,36,41,45,49,57,59,64},
	row DBI/.list={10,20,25,29,32,36,40,46,52,56,59,64},
	row s/.list={10,16,25,29,32,38,40,45,49,55,59,68},
	column addvline/.style={
	every col no #1/.style={
	column type/.add={}{|}}
    },
    column type=r,
	column addvline/.list={2,8},
	every head row/.style={
	before row={
	\caption{Clustering evaluations for real data} \label{tab:real_data_eval_clust} \\
	\toprule
	&  &   & \multicolumn{6}{c|}{extrinsic measurements}& \multicolumn{3}{c}{intrinsic measurements}\\
	},
	after row={
% 	&  &  &  & (rounded) &  (\si{\second}) & (rounded) & (\si{\second}) & \% &  &  &  
	\endfirsthead
	\midrule}
	},
	every last row/.style={after row=\bottomrule}
	]{\data} % filename/path to file
	% }

==> Exact clustering with SOS-SDPA_arxiv/real_data_summary_tab.tex <==
\pgfplotstableread[col sep=comma]{real_data_summary.tex}\data
	\pgfplotstabletypeset[
	font=\footnotesize,
	multicolumn names, % allows to have multicolumn names
	columns={name,type,n,m,K,M},
	fixed zerofill,
	fixed,
 	columns/name/.style={string type,
		column name={instances}
	},
	columns/type/.style={string type,
		column name={type}
	},
	columns/m/.style={int detect,
		column name={$m$},
	},
    columns/n/.style={int detect,
		column name={$n$},
	},
	columns/K/.style={int detect,
		column name={$k_{true}$},
	},
	columns/M/.style={string type,
		column name={measuring type},
	}, 
	    column type=r,
	every head row/.style={
	before row={
	\caption{Summarized information for real data} \label{tab:real_data_sum} \\
	\toprule
% 	&  &  \multicolumn{6}{c|}{extrinsic measurements}& \multicolumn{3}{c}{intrinsic measurements}\\
	},
	after row={
% 	&  &  &  & (rounded) &  (\si{\second}) & (rounded) & (\si{\second}) & \% &  &  &  
	\endfirsthead
	\midrule}
	},
	every last row/.style={after row=\bottomrule}
	]{\data} 
	
	

==> artificial_data_summary.tex <==
name,type,n,m,K, M
3-spiral,artificial,312,3,3, numerical
3MC,artificial,400,3,3, numerical
blobs,artificial,300,3,3, numerical
flame,artificial,240,3,3, numerical
gaussians1,artificial,100,3,2, numerical
insect,artificial,30,4,3, numerical
jain,artificial,373,3,2, numerical
lsun,artificial,400,3,3, numerical
pathbased,artificial,300,3,3, numerical
zelnik1,artificial,299,3,3, numerical
zelnik2,artificial,303,3,3, numerical
zelnik6,artificial,238,3,3, numerical

==> artificial_data_summary_all_label_clust_eval.tex <==
dataname,k,opt_sos_sdp,normalized_mutual_info_score,mutual_info_score,homogeneity_score,fowlkes_mallows_score,completeness_score,adjusted_rand_score,adjusted_mutual_info_score,calinski_harabasz_score,davies_bouldin_score,silhouette_score
3-spiral,3.0,30109.350350293127,1.0,1.09839564632427,1.0,1.0,1.0,1.0,1.0,5.797852185441633,5.882022552277643,0.0013442973442779
3-spiral,2.0,19577.3,0.0009328955978473,0.0008355749515184,0.0007607231094866,0.4044833947646889,0.0012058015309933,-0.0031886440583456,-0.0026783716457486,184.66433452888432,1.168152962826578,0.3480876615461452
3-spiral,3.0,12286.9,0.0005112830235959,0.0005614493915305,0.0005111540576561,0.3275926899333746,0.0005114120546293,-0.005874151386097,-0.0054089048486768,238.3129233311469,0.884839446512841,0.3602912839819129
3-spiral,4.0,9200.4,0.0026194124162049,0.003254053151893,0.0029625510286594,0.2827842205353122,0.0023475110462869,-0.0050653629758994,-0.0052464948632868,245.93028258579045,0.8785236009097113,0.3543972875897688
3-spiral,5.0,7352.09,0.0064345040046559,0.0086788750617078,0.0079014106535758,0.2566357692124038,0.0054269787039899,-0.0022495671885655,-0.0032306153528088,249.36326257951583,0.889096006582799,0.3467646558672821
3MC,3.0,2056.336029450354,1.0,1.079870587934092,1.0,1.0,1.0,1.0,1.0,628.0489014193492,0.7076334829953922,0.4956142510948985
3MC,2.0,3204.77,0.4492228686363406,0.3981389737408716,0.3686913767163101,0.6126015252672271,0.5747663246293778,0.3283870126024342,0.4476566547666701,665.3804951049577,0.7242621893125113,0.5317451487655634
3MC,3.0,1929.39,0.8088691368366148,0.8788705592783972,0.8138665587325336,0.8682238227217552,0.8039327121910247,0.800264438809702,0.8079792049412197,682.4342519561616,0.7032848636744014,0.503592712829231
3MC,4.0,1221.71,0.7291369396590458,0.8957391961817014,0.8294875387756846,0.7303487823449379,0.6504465464055365,0.6070850142928569,0.727458016882152,793.1390215212372,0.7097562688818153,0.4935811979304618
3MC,5.0,786.808,0.7620462130315269,1.0156659897878242,0.9405441736596436,0.7543020207446631,0.6404925281766825,0.6365931123788192,0.7602270163151567,975.9086777188984,0.6328629570160211,0.5254332576187837
blobs,3.0,149.58362626275363,1.0,1.0986122886681091,1.0,1.0,1.0,1.0,1.0,575.4294853200782,0.607849845884483,0.5448276995403188
blobs,2.0,337.014,0.58014076123848,0.5130846366030858,0.4670297628157049,0.7178464751213609,0.7655513902623196,0.4954620872105025,0.5785408945824253,346.7956679706255,0.7930103565086946,0.4831007301050531
blobs,3.0,144.77,0.8616213640770951,0.946544591906397,0.8615820173046946,0.9351244029785276,0.8616607144434407,0.9030061261184824,0.8607687905808963,599.5022773042637,0.5937411887518809,0.559522406348139
blobs,4.0,123.004,0.7649005596468567,0.9363669477900084,0.8523179263953098,0.8378071194534666,0.6937469132566524,0.7628371840809773,0.7629400163807599,486.2641876513297,0.8445585584294051,0.4596767965245963
blobs,5.0,105.468,0.6973676167522715,0.9318293362395388,0.8481876143668774,0.7383789065439691,0.5920861543953757,0.6228084107360515,0.6942709012234543,436.1628497272959,0.977027369372981,0.3628953795527692
flame,2.0,3543.5300833896777,1.0,0.654843055442027,1.0,1.0,1.0,1.0,1.0,110.39059785543064,1.1605356766266266,0.3284556923027034
flame,2.0,3123.77,0.3987957374536851,0.2685370288304292,0.410078455591414,0.7363906803426874,0.3881172502537466,0.4534129232216995,0.3969167583837185,157.20621184586793,1.115414499722493,0.3784940710795816
flame,3.0,1913.55,0.4862702494211092,0.421887845243327,0.6442579511796879,0.7037862995686953,0.3905081610155974,0.4615695027134954,0.4837665868329622,202.7214129395292,0.799521740580789,0.4120656817418855
flame,4.0,1211.45,0.5401951313617974,0.5423000184997735,0.8281373895516299,0.6713416323651232,0.4008278323502659,0.4296731714964762,0.5372775422796912,258.16406743385016,0.6955953710582403,0.4426011973843992
gaussian1,2,0.607786784602029,1.0,0.6931471805599458,1.0,1.0,1.0,1.0,1.0,2000.6559204985397,0.19115128249343344,0.8613276990526753
gaussian1,2,0.607787,1.0,0.6931471805599458,1.0,1.0,1.0,1.0,1.0,2000.6559204985397,0.19115128249343344,0.8613276990526753
gaussian1,3,0.450486,0.8029784244290346,0.6931471805599458,1.0,0.8668497975016037,0.6708136601848828,0.7533010626414229,0.8006130337815637,1352.7850820752535,0.6940085469376062,0.6254060096221804
gaussian1,4,0.336638,0.6822742828433005,0.6931471805599457,0.9999999999999999,0.7329003050503234,0.5177665381802417,0.5396406223089729,0.6773693648790168,1205.2383930182614,0.9463542134292653,0.3791063656428615
insect,3.0,7671.200000000002,1.0,1.0986122886681096,1.0,1.0,1.0,1.0,1.0,45.770922411096016,0.8261096696425358,0.3895558522669933
insect,2.0,10683.5,0.5714653581432843,0.506210859163194,0.4607729809548126,0.6920827420915049,0.7521576281325172,0.4680581910183428,0.5532686294745759,60.27075259031997,0.5799482315693878,0.5487736943919346
insect,3.0,6002.75,0.6449126680040378,0.7053771852381958,0.6420619835714308,0.739971420144161,0.647788778776089,0.6210196944597828,0.6188196252675324,62.245133480488114,0.6953071628687374,0.4687681249232857
insect,4.0,4236.08,0.608739437554484,0.7529275783523527,0.6853442166254631,0.6024640760767093,0.5475380311755307,0.4506480558325025,0.567532700638249,60.23961599748195,0.7966716127699024,0.4367901247098583
insect,5.0,3075.25,0.6225083430893742,0.8194198139949896,0.7458680577735064,0.6125306510286749,0.5341627402160611,0.4690392923266817,0.5691211202622894,62.19958404465761,0.6300622543768848,0.494629899471638
jain,2,29856.32807886973,1.0,0.573112993765099,1.0,1.0,1.0,1.0,1.0,279.48312216168654,0.8996694938176657,0.40246004427612914
jain,2,22208.8,0.36557366684627635,0.23116584276216418,0.40335125058586924,0.6977229525630237,0.33426650953158143,0.3180937556197384,0.36421819127351646,503.4754674444723,0.783072419818396,0.49508103615678445
jain,3,12650.1,0.364735042844682,0.3039508997765924,0.5303507390048328,0.6091264821881899,0.2779408456210691,0.26254177264068607,0.36266884818536577,580.5550521784285,0.6975972408412426,0.4865910776769234
jain,4,8763.07,0.41356869205044755,0.3977188212155168,0.6939623172782735,0.5761813788589303,0.2945546646443085,0.25209632732790277,0.4110797620348116,611.7632259389032,0.792489594238666,0.47945975995143336
lsun,3.0,449.41446954502993,1.0,1.0397207708399177,1.0,1.0,1.0,1.0,1.0,384.4387306734788,0.7089983903842373,0.4774564120231758
lsun,2.0,670.265,0.6491389545399219,0.5611197584224346,0.5396831285472399,0.8181307280119151,0.8142889578784085,0.6660385013251185,0.6481154029375052,385.6928321259544,0.936232660872166,0.4606180392796291
lsun,3.0,381.646,0.5400568656616177,0.5655071130232259,0.5439028716973618,0.6423892311282245,0.5362648689101579,0.4358084271876845,0.5378309512789192,487.9512441770458,0.761378721589555,0.4967022054099482
lsun,4.0,202.504,0.7222378729708145,0.8648766312254383,0.8318354845664621,0.7254440500031895,0.6381580310742303,0.5868596025789136,0.7204692059389957,728.3004198673977,0.5579387214345408,0.5655319907213792
lsun,5.0,143.899,0.8040765861704536,1.039720770839918,1.0000000000000002,0.7712101533765884,0.6723478919069458,0.6477916751094491,0.8025284399220705,806.9620443446847,0.5826937708312114,0.5666015023842174
pathbased,3.0,22689.190096315666,1.0,1.0960106146053783,1.0,1.0,1.0,1.0,1.0,51.90716154797278,2.5279577241776545,0.260827350983948
pathbased,2.0,13638.3,0.4909971532293818,0.4392356920521657,0.4007586114577127,0.6519055872239359,0.6336831547050913,0.3989713297894657,0.4890804951430663,371.0553030050826,0.7522586238450906,0.5150123044043785
pathbased,3.0,8957.91,0.5458430500422186,0.5620602381069193,0.512823717778765,0.6616839023616249,0.5834070523255318,0.4613289348654503,0.5428393181773931,359.10473171402344,0.6692535513389878,0.5419218557223351
pathbased,4.0,7230.33,0.4658578423230228,0.5496313607454874,0.5014836110354494,0.580607790951345,0.4349580956992332,0.3827734541613792,0.4612180471591813,319.1811337346417,0.8696701159591098,0.4352170786214091
pathbased,5.0,5901.86,0.4666431283706784,0.5981987867410505,0.545796526757575,0.5838176774556085,0.4075401699442199,0.4076167756503255,0.460928129070025,308.8800396373083,0.9428932950905058,0.3825725727537546
zelnik1,3,13.50248673323875,1.0,1.0463564577282705,1.0,1.0,1.0,1.0,1.0,0.014217517052841574,120.43118334004778,-0.010563524873156782
zelnik1,2,9.60258,0.12186112054419279,0.103248340258415,0.09867415592060855,0.4602705429856286,0.15929249721219604,0.02615527060591208,0.11835050146180513,120.66118216909004,1.3011778495789665,0.30622537731244953
zelnik1,3,6.88992,0.1621105715363804,0.16899227096214928,0.16150545037878009,0.4030883988072931,0.1627202442274319,0.05330698323782812,0.15663535783669041,142.07033597185406,1.0628037616106143,0.3273632309615051
zelnik1,4,5.48487,0.2052404753362546,0.24356706913062656,0.23277638067951675,0.3881516397256538,0.1835300813021801,0.0993537434579592,0.19836296340096374,143.76413641071147,1.0732411603047478,0.32553395341276403
zelnik1,5,4.14001,0.38481469008921537,0.47284648160580967,0.4518980870366107,0.46124294710352826,0.33507365422744406,0.20297872393034727,0.37786636674666907,166.24032659730273,0.8420161038120229,0.39752307176738416
zelnik2,3,27.21008027054806,1.0,1.0975939420343654,1.0,1.0,1.0,1.0,1.0,50.53473179960157,2.2837843856324795,0.4692214114072803
zelnik2,2,18.8778,0.5035596810686214,0.4508601731442408,0.4107713753490491,0.6651722410068127,0.6504997357372246,0.42096401946901046,0.5017106628316834,279.02146941811594,0.6981217369734207,0.5749904584972232
zelnik2,3,11.8813,0.5463765765707048,0.5537671932724482,0.5045282887094413,0.6726050010685936,0.5957950174263004,0.4708785919450187,0.5433510431307448,309.2557998452903,0.6032329891280371,0.6322744873259036
zelnik2,4,8.68286,0.556547659042638,0.6040810733233957,0.550368447008504,0.6765081658527577,0.5628671996937633,0.4937406137101005,0.5523355426870863,317.88997412340456,0.5886644441624687,0.6536244570141765
zelnik2,5,6.37043,0.6113245263886611,0.7225693687305899,0.6583212070133367,0.7101001750745403,0.5705908032997264,0.5654820896922822,0.6067883724773538,350.9179183446262,0.6020361202471877,0.6824724738526461
zelnik6,3,6.0499989559164025,1.0,1.0719022217569947,1.0,1.0,1.0,1.0,1.0,191.4378235419437,1.5564445962690894,0.5749826418958833
zelnik6,2,3.80238,0.5979727711023263,0.5266688268014077,0.49134036305860557,0.7664423540430446,0.7637173981526055,0.5821826429846935,0.59602789846613,751.2905120512687,0.3519045622593329,0.7348068903877594
zelnik6,3,2.49599,0.6400618519311038,0.6248330276145528,0.5829197989629743,0.7915155418959071,0.7096244161981063,0.6483717070239138,0.636822029675717,631.3318427553139,0.5120883365552338,0.7371089795591736
zelnik6,4,1.37484,0.6733330764904996,0.7092776134836439,0.6616999191596419,0.8178682551332983,0.6853825921323213,0.705791595796343,0.6691589254118446,824.4668082737813,0.42392184952718037,0.7599966725533781
zelnik6,5,1.07112,0.6835882968102652,0.751594176677411,0.7011779259543329,0.8301868975785732,0.6668595720051071,0.7307789007864689,0.6782580684682645,806.8097010845635,0.47163075434077983,0.73735109102075



==> artificial_data_summary_clust_eval.tex <==
dataname,k,opt_sos_sdp,true_k,normalized_mutual_info_score,mutual_info_score,homogeneity_score,fowlkes_mallows_score,completeness_score,adjusted_rand_score,adjusted_mutual_info_score,calinski_harabasz_score,davies_bouldin_score,silhouette_score,
3-spiral,2.0,19577.3,0,0.0009328955978473127,0.0008355749515184253,0.0007607231094866753,0.4044833947646889,0.001205801530993308,-0.003188644058345625,-0.0026783716457486444,184.66433452888432,1.1681529628265779,0.34808766154614523,
3-spiral,3.0,12286.9,1,0.0005112830235959982,0.0005614493915305219,0.0005111540576561699,0.3275926899333746,0.0005114120546293565,-0.005874151386097084,-0.005408904848676883,238.3129233311469,0.884839446512841,0.36029128398191296,
3-spiral,4.0,9200.4,0,0.002619412416204974,0.0032540531518930327,0.0029625510286594545,0.2827842205353122,0.002347511046286977,-0.005065362975899442,-0.005246494863286878,245.93028258579045,0.8785236009097113,0.35439728758976885,
3-spiral,5.0,7352.09,0,0.006434504004655965,0.008678875061707891,0.007901410653575825,0.25663576921240383,0.00542697870398998,-0.002249567188565553,-0.0032306153528088503,249.36326257951583,0.8890960065827991,0.34676465586728217,
3MC,2.0,3204.77,0,0.44922286863634064,0.3981389737408716,0.3686913767163101,0.6126015252672271,0.5747663246293778,0.3283870126024342,0.44765665476667016,665.3804951049577,0.7242621893125113,0.5317451487655634,
3MC,3.0,1929.39,1,0.8088691368366148,0.8788705592783972,0.8138665587325336,0.8682238227217552,0.8039327121910247,0.8002644388097021,0.8079792049412197,682.4342519561617,0.7032848636744014,0.503592712829231,
3MC,4.0,1221.71,0,0.7291369396590458,0.8957391961817014,0.8294875387756846,0.7303487823449379,0.6504465464055365,0.6070850142928569,0.727458016882152,793.1390215212372,0.7097562688818153,0.4935811979304618,
3MC,5.0,786.808,0,0.7620462130315269,1.0156659897878242,0.9405441736596436,0.7543020207446631,0.6404925281766825,0.6365931123788192,0.7602270163151567,975.9086777188983,0.6328629570160211,0.5254332576187837,
blobs,2.0,337.014,0,0.58014076123848,0.5130846366030858,0.467029762815705,0.7178464751213609,0.7655513902623196,0.4954620872105026,0.5785408945824253,346.7956679706255,0.7930103565086946,0.4831007301050532,
blobs,3.0,144.77,1,0.8616213640770951,0.9465445919063971,0.8615820173046946,0.9351244029785276,0.8616607144434407,0.9030061261184824,0.8607687905808963,599.5022773042638,0.5937411887518809,0.5595224063481391,
blobs,4.0,123.00399999999999,0,0.7649005596468567,0.9363669477900084,0.8523179263953098,0.8378071194534666,0.6937469132566524,0.7628371840809773,0.7629400163807599,486.2641876513297,0.8445585584294051,0.4596767965245963,
blobs,5.0,105.46799999999999,0,0.6973676167522715,0.9318293362395388,0.8481876143668774,0.7383789065439691,0.5920861543953757,0.6228084107360515,0.6942709012234543,436.16284972729585,0.9770273693729808,0.3628953795527693,
flame,2.0,3123.77,1,0.3987957374536851,0.2685370288304292,0.4100784555914141,0.7363906803426874,0.3881172502537466,0.4534129232216995,0.39691675838371854,157.2062118458679,1.115414499722493,0.3784940710795816,
flame,3.0,1913.55,0,0.4862702494211093,0.4218878452433271,0.6442579511796879,0.7037862995686953,0.39050816101559743,0.4615695027134954,0.4837665868329622,202.7214129395292,0.799521740580789,0.4120656817418856,
flame,4.0,1211.45,0,0.5401951313617974,0.5423000184997735,0.8281373895516299,0.6713416323651232,0.4008278323502659,0.4296731714964762,0.5372775422796912,258.16406743385016,0.6955953710582403,0.4426011973843992,
flame,5.0,1022.72,0,0.5256495878511207,0.5889556160037883,0.8993843808975512,0.6050194209391393,0.3713407501938503,0.3477673085111003,0.5220412914409845,239.22155721975062,0.8354291986139307,0.40290334974973696,
insect,2.0,10683.5,0,0.5714653581432843,0.506210859163194,0.4607729809548126,0.6920827420915049,0.7521576281325172,0.4680581910183429,0.5532686294745759,60.270752590319965,0.5799482315693878,0.5487736943919346,
insect,3.0,6002.75,1,0.6449126680040378,0.7053771852381958,0.6420619835714308,0.7399714201441608,0.647788778776089,0.6210196944597828,0.6188196252675324,62.24513348048811,0.6953071628687417,0.4687681249232857,
insect,4.0,4236.08,0,0.608739437554484,0.7529275783523527,0.6853442166254631,0.6024640760767093,0.5475380311755307,0.4506480558325025,0.567532700638249,60.239615997481955,0.7966716127699024,0.4367901247098583,
insect,5.0,3075.25,0,0.6225083430893742,0.8194198139949896,0.7458680577735064,0.6125306510286749,0.5341627402160611,0.4690392923266817,0.5691211202622894,62.19958404465761,0.6300622543768848,0.4946298994716379,
lsun,2.0,670.265,0,0.6491389545399219,0.5611197584224346,0.5396831285472399,0.8181307280119151,0.8142889578784085,0.6660385013251185,0.6481154029375052,385.69283212595434,0.9362326608721658,0.4606180392796291,
lsun,3.0,381.64599999999996,1,0.5400568656616177,0.5655071130232259,0.5439028716973618,0.6423892311282245,0.5362648689101579,0.4358084271876845,0.5378309512789192,487.9512441770458,0.761378721589555,0.4967022054099482,
lsun,4.0,202.50400000000002,0,0.7222378729708145,0.8648766312254383,0.8318354845664621,0.7254440500031895,0.6381580310742303,0.5868596025789136,0.7204692059389957,728.3004198673977,0.5579387214345408,0.5655319907213792,
lsun,5.0,143.899,0,0.8040765861704536,1.039720770839918,1.0000000000000002,0.7712101533765884,0.6723478919069458,0.6477916751094491,0.8025284399220705,806.9620443446847,0.5826937708312114,0.5666015023842174,
pathbased,2.0,13638.3,0,0.4909971532293818,0.4392356920521657,0.4007586114577128,0.6519055872239359,0.6336831547050913,0.3989713297894657,0.4890804951430663,371.05530300508264,0.7522586238450906,0.5150123044043785,
pathbased,3.0,8957.91,1,0.5458430500422186,0.5620602381069193,0.512823717778765,0.6616839023616249,0.5834070523255318,0.4613289348654504,0.5428393181773931,359.10473171402344,0.6692535513389878,0.5419218557223351,
pathbased,4.0,7230.33,0,0.4658578423230228,0.5496313607454874,0.5014836110354494,0.580607790951345,0.4349580956992333,0.3827734541613793,0.4612180471591814,319.18113373464166,0.8696701159591098,0.4352170786214091,
pathbased,5.0,5901.86,0,0.4666431283706784,0.5981987867410505,0.545796526757575,0.5838176774556085,0.4075401699442199,0.4076167756503256,0.460928129070025,308.8800396373083,0.9428932950905058,0.3825725727537546,


==> real_data_summary.tex <==
name,type,n,m,K, M
dermatology,real,358,35,6, mixed
ecoli,real,336,8,8,numerical
glass,real,214,10,7, numerical
haberman,real,306,4,2, numerical
heart-statlog,real,270,14,2, mixed
iono,real,351,35,2, numerical
iris,real,150,5,3, numerical
sonar,real,208,61,2, numerical
tae,real,151,6,3, mixed
thy,real,215,6,3, numerical 
wine,real,178,14,3, numerical
%wisc,real,699,10,2
zoo,real,101,17,7, categorical


==> real_data_summary_all_label_clust_eval.tex <==
dataname,k,opt_sos_sdp,normalized_mutual_info_score,mutual_info_score,homogeneity_score,fowlkes_mallows_score,completeness_score,adjusted_rand_score,adjusted_mutual_info_score,calinski_harabasz_score,davies_bouldin_score,silhouette_score
arrhythmia,3.0,16621623.2990983,1.0,1.664514143432401,1.0,1.0,1.0,1.0,1.0,7.3538326473514335,3.99676672946264,-0.0250518944110154
arrhythmia,2.0,17873000.0,0.0311133712137884,0.0363669388011164,0.0218483807690116,0.4239995598434332,0.0540217511950851,0.023554266039522,0.0187408106998119,52.61608034768564,2.654391799943445,0.1261106391687146
arrhythmia,3.0,16838500.0,0.1296017009246813,0.1666980831688465,0.1001481926882866,0.4287654161535796,0.1835976243131432,0.0817991547272355,0.1096691986306355,41.65533164260298,2.532531179757959,0.0976110690661389
arrhythmia,4.0,15929100.0,0.1602572886316708,0.2201493289433538,0.1322604135338754,0.4378424830046956,0.2032896215126699,0.1273054528652708,0.1336420160051497,37.81602509175721,2.3000398622870994,0.0951958714299945
arrhythmia,5.0,15241000.0,0.1625611349497498,0.2523178570154988,0.1515864902746895,0.3644819235477951,0.1752489045074288,0.1053165712552402,0.1305508149498917,34.62150334727939,2.4259279061575683,0.0763140260241946
arrhythmia,6.0,14588400.0,0.1702231406769618,0.2660839897923807,0.1598568512272823,0.3667281236518344,0.1820271122876649,0.1098105634875947,0.1356665090835094,32.861907093261394,2.1046638720575146,0.0785622856050936
arrhythmia,7.0,13955400.0,0.1896998322294754,0.3008503889776913,0.1807436663513754,0.3653351146137732,0.1995898600825743,0.1100530620563422,0.151059984856815,31.926916875762117,1.9796163874290629,0.0893736745008537
balance-scale,3.0,,1.0,0.91364855987124,1.0,1.0,1.0,1.0,1.0,63.395442099716654,4.218747293065079,0.0888307913921624
balance-scale,2.0,4062.5,0.0533186532336323,0.0428352393431122,0.046883715713566,0.5041814760723365,0.061801040527784,0.0758211964357062,0.0514170465731192,143.76923076923077,2.01857949405675,0.1819410926722415
dermatology,6.0,71575.45485344502,1.0,1.6832739364924156,1.0,1.0,1.0,1.0,1.0,20.679657647590588,5.89901002547441,-0.0335783541649112
dermatology,4.0,16162.4,0.0837777622186428,0.1269530274813306,0.0754203013122592,0.2526072253328422,0.0942182590471259,0.0276453102830479,0.070566805693841,558.0661308282387,0.8923486314414688,0.3489327873326072
dermatology,5.0,13364.9,0.1095777420570606,0.1766180225193485,0.1049252998518963,0.2394009308147556,0.1146619106332565,0.0354501534209339,0.0932367382420944,523.1991232483508,0.9420232132816876,0.3192755968323302
dermatology,6.0,11698.0,0.1077224207166259,0.183017909029585,0.1087273467864389,0.2157509523425433,0.1067359008345187,0.0265942727992582,0.0880755985488046,486.8794773046705,1.0589993360439955,0.2864864243102078
dermatology,7.0,10552.3,0.1048528806488991,0.1879476552808499,0.1116560122546023,0.1979203758764419,0.0988311593782073,0.0281374558429034,0.0822901312897753,454.8607809904705,1.207820098125675,0.2598450604236552
dermatology,8.0,9831.41,0.1772437187904006,0.3290176844917573,0.195462947152476,0.2181678945846156,0.1621313502430022,0.0630829923519399,0.1536292513311843,420.94172423979455,1.2225216095179965,0.2613383722102094
ecoli,8.0,21.306504120879126,1.0,1.517122829952031,1.0,1.0,1.0,1.0,1.0,81.17586758649125,1.5753319355303452,0.2382407258501354
ecoli,6.0,16.5347,0.621433531799543,0.9901249222167764,0.652633328474849,0.6165667143315855,0.5930807083894373,0.4936599210527242,0.6083844151951374,166.38453535988808,1.264422122110093,0.2809992948229829
ecoli,7.0,15.0043,0.6237586989449899,1.0293283922625398,0.6784739982425059,0.6418754378490984,0.5772098144799364,0.5265993900048032,0.6089821609647691,157.92598780623803,1.229209297964023,0.2734487842081349
ecoli,8.0,13.848,0.6162561974225754,1.0753129421737673,0.708784365342236,0.5605420133404836,0.54509662540823,0.426192978871245,0.5996568042730128,150.13386710651346,1.2212185354020693,0.2540869241157364
ecoli,9.0,12.9786,0.6504800716742517,1.1524170933524711,0.7596069814524568,0.5758129991080211,0.5687693420588131,0.4435754287012778,0.6338409588866849,142.47844313205275,1.1624952775469637,0.2649987522623291
ecoli,10.0,12.2649,0.6557502472519027,1.16832132641489,0.770090135979188,0.576594900482865,0.5709742805737514,0.4444173551129747,0.6380161381587897,135.71435262960037,1.1207675015930014,0.270912320776119
glass,6.0,911.2040712197261,1.0,1.5086584002236936,1.0,1.0,1.0,1.0,1.0,19.702067127104986,3.73631979010432,-0.0914413867182059
glass,5.0,400.259,0.3772224403230368,0.5043250206736848,0.3342870861945334,0.4978578683426982,0.4328122216009364,0.2520460591021136,0.3532086463841432,123.03415777775744,0.9042043494669332,0.4426886725031028
glass,6.0,336.061,0.4157375276959366,0.5707364427990196,0.3783072713573826,0.4986501147071163,0.4613878987846299,0.255213359620384,0.3879403868556083,124.61616247195136,0.9350845435798436,0.4468862914963273
glass,7.0,292.254,0.4242314831428778,0.6024588284534091,0.3993341556737301,0.4976789511947704,0.4524397932313275,0.267756636335495,0.3928546495972367,124.00967694153962,0.8741233438503606,0.4550617511042344
glass,8.0,266.496,0.4539089159703398,0.6571087899089563,0.4355583674949376,0.5073453178437526,0.4738737325107051,0.2792875315533171,0.4197452779369728,118.84939171483424,0.8579717871319198,0.4574789512940245
glass,9.0,245.351,0.4084028991390969,0.6664680570982393,0.4417620695310615,0.4075664886202422,0.3797281509776367,0.2224588792384759,0.3706311820149561,114.61555420318405,0.9710525084978392,0.3041441401748521
haberman,2.0,53123.17333333333,1.0,0.5779217946828967,1.0,1.0,1.0,1.0,1.0,8.360345155772595,4.725836847244438,0.0597219507631459
haberman,2.0,30507.0,7.965736046142885e-05,5.050237119169632e-05,8.7386168260719e-05,0.5519976954266277,7.318460028939525e-05,-0.0018130326610555,-0.0025219560050244,239.92636004273905,0.9687879726138507,0.4012977121920988
haberman,3.0,21164.6,0.0361368231690338,0.0274498400271737,0.0474974992805649,0.5319055614762077,0.0291617727025833,0.0522418524106729,0.0319025371591291,239.22305793227412,0.8473812792396576,0.4316143935765462
haberman,4.0,15366.5,0.0225034689759232,0.0210744260091325,0.0364658786068034,0.4365966353327911,0.0162727864971384,0.0273170705144174,0.0172778467931294,256.9162536550288,0.8533987498306269,0.3719096040767244
heart-statlog,2.0,934653.3878499997,1.0,0.6869615765973238,1.0,1.0,1.0,1.0,1.0,11.137445285462835,4.156427207730943,0.0501465917975156
heart-statlog,2.0,549315.0,0.0199122924571302,0.0134400738960099,0.0195645205698136,0.5307324925591533,0.0202726518312902,0.0302303325860961,0.017199186261725,206.9495407269051,0.9871370082638804,0.3804182800071519
heart-statlog,3.0,431736.0,0.0139079599739712,0.0121248819526923,0.0176500147399067,0.4312904396637974,0.0114750795137229,0.0106123234232289,0.0096650455661279,167.52135434182202,1.1633560674055936,0.2773423952865388
heart-statlog,4.0,351403.0,0.025088024444836,0.0231136120846906,0.0336461497587355,0.4213882389610534,0.0200007090790926,0.0228636819864862,0.0188163950819586,156.96769726829186,1.0773743172759558,0.2754035733026458
iono,2.0,3086.176177564397,1.0,0.6528257939163475,1.0,1.0,1.0,1.0,1.0,17.74606012127195,4.08644491721087,0.1548790250623376
iono,2.0,2419.36,0.13485692093441,0.0905264814101238,0.1386686651381361,0.6052850553774272,0.1312491260868341,0.177606854737686,0.1330081904044343,118.82649338303231,1.513475950743014,0.2959701497777325
iono,3.0,2193.32,0.192828707888386,0.1569871352216589,0.240473242149153,0.587003830812214,0.1609416299929337,0.2200462194832898,0.1899676707646518,83.28120876024403,1.8019594860993509,0.2884590817381463
iono,4.0,1999.18,0.2380034420870625,0.2194422392554498,0.3361421091207204,0.5775331551770819,0.1842194805618035,0.2437927008085461,0.2344108128480203,71.96981929435267,1.7104687629047608,0.3057357408709429
iris,3.0,89.38680000000001,1.0,1.0986122886681096,1.0,1.0,1.0,1.0,1.0,486.3208393185568,0.7517428073901344,0.5032506980366628
iris,2.0,152.369,0.6565191143081124,0.5738298777087831,0.5223224641010155,0.7504732564880243,0.8835142349190769,0.5399218294207123,0.6538380713762781,513.3038433517569,0.4048341363918284,0.680813620271351
iris,3.0,78.9408,0.7581756800057784,0.8255910976103356,0.7514854021988338,0.8208080729114153,0.7649861514489815,0.7302382722834697,0.7551191675800485,560.3999242466399,0.6623228649898628,0.552591944521368
iris,4.0,57.3179,0.7219203867820961,0.8880235203213085,0.8083138423637095,0.7565926353252695,0.6522113355514313,0.6498176853819967,0.7172081944051022,529.3982941434153,0.780640036237599,0.4978256900754499
iris,5.0,46.5356,0.6938628345588717,0.9051279136224294,0.8238829320940431,0.7254830776265845,0.59928706467119,0.6078964652364223,0.6872109247445372,494.0943819140987,0.80624149219652,0.4885175508538638
sonar,2.0,351.5856632023387,1.0,0.690880304410466,1.0,1.0,1.0,1.0,1.0,6.004452460055308,5.685775044966328,0.0301424569014513
sonar,2.0,280.534,0.0087901130807924,0.0060755607287341,0.0087939411356045,0.5027663757107326,0.0087862883572801,0.0064098447858296,0.0053052470002705,59.699458265423424,1.8005189338588006,0.1983999469666345
sonar,3.0,235.04,0.0031105584580843,0.0027476044649865,0.0039769616349551,0.4143222590518839,0.0025541275810736,-0.0017586922582194,-0.0024019487046078,55.29428177572339,1.6929144859460152,0.1924868838776389
sonar,4.0,217.165,0.0232080086074249,0.0233604906702342,0.0338126452890678,0.3853278410759623,0.0176670910080888,0.0205020854733452,0.0160545336776992,45.29926475510734,1.907214357311025,0.173614025494858
tae,3.0,38345.79758241758,1.0,1.0983062060529227,1.0,1.0,1.0,1.0,1.0,1.975107479601828,9.1301455401467,-0.0191986930578776
tae,2.0,21803.3,0.0070823307737267,0.0062585814620781,0.0056983939702664,0.414028536176009,0.0093541109382047,0.0001139684162335,-0.0005244138766196,120.04262044283244,1.0472127358490746,0.3801283934670079
tae,3.0,16775.4,0.0263141921557827,0.027684818359896,0.0252068304880015,0.3619355927406001,0.0275233195406774,0.0088791124595939,0.013589272548773,99.66676208871986,1.1042788462657311,0.3374766558094673
tae,4.0,13221.3,0.0381660879455284,0.0460054335294892,0.041887620479559,0.3111809990024711,0.0350518810681581,0.0079944491521073,0.0215936711539228,96.90851752548882,1.103668339637843,0.3432389497757682
tae,5.0,10537.7,0.0461049400266953,0.0612875787555209,0.0558019051679362,0.2779161092756532,0.0392792040381583,0.0141953136972677,0.0260880765325214,99.86594938807347,0.9866865681764873,0.3643123596056096
thy,3.0,38859.19328571429,1.0,0.8214826899116975,1.0,1.0,1.0,1.0,1.0,68.80148036158958,1.2444333530707423,0.3835002853016623
thy,2.0,41608.0,0.1276326688305902,0.0966408677875019,0.1176420014375349,0.5372099535501407,0.1394777198380171,0.0477515733517705,0.1221508130975099,115.04657594115812,1.0656984721770733,0.3462207447643413
thy,3.0,28560.2,0.4945160467056619,0.3986646698203863,0.4852989292607485,0.8062522135438603,0.5040900576587282,0.5790671581240897,0.4882857152795125,131.83643925618364,0.923577781311556,0.4565740832904507
thy,4.0,20082.7,0.3211378902629165,0.3032556869761809,0.3691565150432791,0.6175825442367808,0.2841735594981179,0.2814179070237005,0.3100305802062995,154.09183040925103,0.8249080653270505,0.4107051556699644
thy,5.0,15402.5,0.3311263808530725,0.3542028607238399,0.4311750753529739,0.5803410290976675,0.2687632789007592,0.275402190922566,0.318149238984441,165.92420027947998,0.8300573416438153,0.3944580789974784
wine,3.0,33788.03886609779,1.0,1.0860384436406825,1.0,1.0,1.0,1.0,1.0,15.81175326135954,2.806900926429026,0.0688642280213505
wine,2.0,4543750.0,0.4259186266746114,0.3629524368591491,0.3341985166219701,0.6590510206234098,0.587027006858955,0.3694075388574537,0.4220526675739516,19.490035043004056,2.176493391527308,0.1139838328809922
wine,3.0,2370690.0,0.4287568597645354,0.4657066646034707,0.4288123199785646,0.5835370218944976,0.4287014138944858,0.3711137182308475,0.4226866642766121,18.638514675777287,4.303568871252648,0.040614246164066
wine,4.0,1331900.0,0.3884332923957888,0.4644628506130969,0.4276670437706578,0.5207343245323419,0.3557931783115363,0.303442531578347,0.3794660493529976,11.956480798763463,7.735705077833749,-0.0318784506667515
wine,5.0,916379.0,0.4109925606542485,0.537739887874978,0.4951389069362355,0.5087079622475457,0.351292227983938,0.3115880103317625,0.4003850916370255,14.735786788755284,5.408027216584347,-0.058420718797689
zoo,7.0,277.96510318949345,1.0,1.657009703742392,1.0,1.0,1.0,1.0,1.0,23.902799308963928,1.8586399351741556,0.3039716264714694
zoo,5.0,158.63,0.6993349994752281,1.0984475727336185,0.6629095594628994,0.680681732167751,0.7399961819075096,0.5811563562389545,0.6707532901380499,82.21871061168216,0.9255466297226396,0.4301899320142995
zoo,6.0,134.773,0.745044183859346,1.235315542067745,0.7455089365365565,0.7363517316948206,0.7445800102777634,0.6610838742714487,0.7159708514353341,79.97448856682449,0.9310474847925786,0.4477971563030443
zoo,7.0,119.704,0.7816625894813721,1.3471139658020228,0.8129789238768711,0.7741355207962075,0.7526694063540147,0.7087529337715824,0.7527195513185745,76.21779577510424,1.0211302587108235,0.4405712903716863
zoo,8.0,109.287,0.8078200013977627,1.4227394115400198,0.8586186359239372,0.787945046988338,0.7626964323306963,0.7251155013659698,0.7790454380030649,72.06147916786657,1.0561214365381415,0.442117718340804
zoo,9.0,100.129,0.8337886459103071,1.5011749300384132,0.90595421779847,0.8072445195129591,0.7722718101398626,0.74711213630809,0.8062558551394664,69.13282029937969,0.9903091219416648,0.4547490257242741


==> real_data_summary_clust_eval.tex <==
dataname,k,opt_sos_sdp,true_k,normalized_mutual_info_score,mutual_info_score,homogeneity_score,fowlkes_mallows_score,completeness_score,adjusted_rand_score,adjusted_mutual_info_score,calinski_harabasz_score,davies_bouldin_score,silhouette_score,
arrhythmia,2.0,17873000.0,0,0.03111337121378848,0.03636693880111641,0.02184838076901168,0.4239995598434333,0.054021751195085135,0.023554266039522005,0.01874081069981196,52.616080347685646,2.6543917999434483,0.12611063916871462,
arrhythmia,3.0,16838500.0,0,0.1296017009246813,0.1666980831688465,0.10014819268828663,0.4287654161535796,0.18359762431314328,0.08179915472723552,0.10966919863063558,41.65533164260298,2.5325311797579544,0.09761106906613894,
arrhythmia,4.0,15929100.0,0,0.16025728863167088,0.22014932894335384,0.13226041353387544,0.4378424830046957,0.20328962151267,0.12730545286527087,0.13364201600514974,37.81602509175721,2.300039862287101,0.0951958714299946,
arrhythmia,5.0,15241000.0,0,0.16256113494974986,0.2523178570154988,0.1515864902746895,0.3644819235477951,0.17524890450742886,0.10531657125524024,0.13055081494989176,34.62150334727939,2.425927906157564,0.0763140260241947,
arrhythmia,6.0,14588400.0,0,0.1702231406769618,0.2660839897923807,0.15985685122728238,0.3667281236518344,0.18202711228766494,0.10981056348759476,0.13566650908350944,32.861907093261394,2.1046638720575164,0.07856228560509364,
arrhythmia,7.0,13955400.0,0,0.18969983222947548,0.3008503889776913,0.18074366635137545,0.3653351146137732,0.19958986008257434,0.11005306205634223,0.15105998485681507,31.926916875762114,1.979616387429061,0.0893736745008538,
balance-scale,2.0,4062.5,0,0.053318653233632315,0.04283523934311223,0.04688371571356603,0.5041814760723365,0.061801040527784075,0.07582119643570624,0.05141704657311922,143.76923076923075,2.01857949405675,0.1819410926722415,
dermatology,4.0,16162.4,0,0.08377776221864286,0.12695302748133064,0.0754203013122592,0.2526072253328422,0.09421825904712597,0.02764531028304793,0.07056680569384108,558.0661308282387,0.8923486314414679,0.34893278733260724,
dermatology,5.0,13364.9,0,0.10957774205706064,0.17661802251934858,0.10492529985189633,0.2394009308147557,0.11466191063325652,0.03545015342093395,0.0932367382420944,523.1991232483508,0.9420232132816873,0.3192755968323302,
dermatology,6.0,11698.0,1,0.10772242071662592,0.18301790902958506,0.10872734678643893,0.21575095234254332,0.10673590083451877,0.02659427279925827,0.0880755985488046,486.8794773046705,1.0589993360439955,0.2864864243102078,
dermatology,7.0,10552.3,0,0.10485288064889917,0.18794765528084995,0.11165601225460238,0.19792037587644196,0.0988311593782073,0.02813745584290346,0.08229013128977533,454.8607809904705,1.207820098125675,0.25984506042365524,
dermatology,8.0,9831.41,0,0.17724371879040066,0.3290176844917573,0.195462947152476,0.21816789458461566,0.16213135024300224,0.06308299235193998,0.15362925133118432,420.94172423979455,1.2225216095179972,0.2613383722102094,
ecoli,6.0,16.5347,0,0.621433531799543,0.9901249222167764,0.652633328474849,0.6165667143315855,0.5930807083894373,0.4936599210527242,0.6083844151951374,166.3845353598881,1.2644221221100922,0.280999294822983,
ecoli,7.0,15.0043,0,0.6237586989449899,1.0293283922625398,0.6784739982425059,0.6418754378490984,0.5772098144799364,0.5265993900048032,0.6089821609647691,157.92598780623803,1.2292092979640221,0.2734487842081351,
ecoli,8.0,13.847999999999999,1,0.6162561974225754,1.0753129421737673,0.708784365342236,0.5605420133404836,0.54509662540823,0.426192978871245,0.5996568042730128,150.13386710651346,1.2212185354020686,0.2540869241157365,
ecoli,9.0,12.9786,0,0.6504800716742517,1.1524170933524711,0.7596069814524568,0.5758129991080211,0.5687693420588131,0.4435754287012778,0.6338409588866849,142.47844313205275,1.162495277546962,0.2649987522623294,
ecoli,10.0,12.2649,0,0.6557502472519027,1.16832132641489,0.770090135979188,0.576594900482865,0.5709742805737514,0.4444173551129748,0.6380161381587897,135.71435262960034,1.1207675015930003,0.2709123207761192,
glass,5.0,400.259,0,0.3772224403230369,0.5043250206736848,0.33428708619453346,0.4978578683426982,0.4328122216009364,0.25204605910211364,0.3532086463841432,123.03415777775743,0.9042043494669558,0.44268867250311705,
glass,6.0,336.061,1,0.41573752769593664,0.5707364427990196,0.3783072713573826,0.4986501147071163,0.4613878987846299,0.25521335962038405,0.3879403868556083,124.61616247195136,0.9350845435798348,0.44688629149634107,
glass,7.0,292.254,0,0.42423148314287773,0.6024588284534091,0.39933415567373015,0.4976789511947705,0.4524397932313275,0.267756636335495,0.3928546495972368,124.00967694153962,0.8741233438503809,0.4550617511042501,
glass,8.0,266.496,0,0.4539089159703398,0.6571087899089563,0.4355583674949377,0.5073453178437526,0.4738737325107051,0.27928753155331715,0.4197452779369728,118.84939171483423,0.8579717871319328,0.4574789512940386,
glass,9.0,245.351,0,0.4084028991390969,0.6664680570982393,0.4417620695310615,0.4075664886202423,0.3797281509776368,0.2224588792384759,0.37063118201495615,114.61555420318405,0.9710525084978312,0.30414414017487085,
haberman,2.0,30507.0,1,7.965736046142884e-05,5.050237119169632e-05,8.738616826071899e-05,0.5519976954266277,7.318460028939525e-05,-0.001813032661055529,-0.0025219560050244805,239.92636004273902,0.9687879726138507,0.4012977121920989,
haberman,3.0,21164.6,0,0.03613682316903384,0.02744984002717371,0.04749749928056498,0.5319055614762077,0.0291617727025833,0.052241852410672925,0.03190253715912912,239.22305793227414,0.8473812792396576,0.4316143935765462,
haberman,4.0,15366.5,0,0.022503468975923268,0.021074426009132518,0.03646587860680349,0.4365966353327911,0.01627278649713847,0.02731707051441749,0.01727784679312943,256.9162536550288,0.8533987498306269,0.3719096040767245,
heart-statlog,2.0,549315.0,1,0.019912292457130217,0.013440073896009984,0.01956452056981369,0.5307324925591533,0.020272651831290223,0.030230332586096142,0.017199186261725025,206.9495407269051,0.9871370082638804,0.3804182800071519,
heart-statlog,3.0,431736.0,0,0.013907959973971276,0.012124881952692318,0.01765001473990671,0.43129043966379743,0.0114750795137229,0.010612323423228943,0.009665045566127932,167.52135434182205,1.163356067405595,0.2773423952865388,
heart-statlog,4.0,351403.0,0,0.02508802444483609,0.023113612084690628,0.03364614975873553,0.42138823896105343,0.020000709079092627,0.022863681986486247,0.018816395081958613,156.9676972682919,1.0773743172759576,0.2754035733026457,
iono,2.0,2419.36,1,0.13485692093441007,0.09052648141012387,0.13866866513813614,0.6052850553774272,0.13124912608683412,0.17760685473768606,0.13300819040443435,118.82649338303233,1.5134759507430142,0.2959701497777326,
iono,3.0,2193.32,0,0.19282870788838605,0.1569871352216589,0.24047324214915305,0.587003830812214,0.16094162999293374,0.22004621948328987,0.18996767076465187,83.28120876024404,1.8019594860993509,0.2884590817381463,
iono,4.0,1999.18,0,0.23800344208706256,0.2194422392554498,0.3361421091207204,0.5775331551770819,0.1842194805618036,0.2437927008085461,0.2344108128480203,71.96981929435267,1.7104687629047608,0.3057357408709429,
iris,2.0,152.369,0,0.6565191143081124,0.5738298777087831,0.5223224641010155,0.7504732564880243,0.8835142349190769,0.5399218294207123,0.6538380713762781,513.3038433517569,0.40483413639182864,0.6808136202713507,
iris,3.0,78.9408,1,0.7581756800057784,0.8255910976103356,0.7514854021988338,0.8208080729114153,0.7649861514489815,0.7302382722834697,0.7551191675800485,560.3999242466399,0.6623228649898673,0.5525919445213676,
iris,4.0,57.3179,0,0.7219203867820961,0.8880235203213085,0.8083138423637095,0.7565926353252695,0.6522113355514313,0.6498176853819967,0.7172081944051022,529.3982941434153,0.7806400362376116,0.4978256900754493,
iris,5.0,46.5356,0,0.6938628345588717,0.9051279136224294,0.8238829320940431,0.7254830776265845,0.59928706467119,0.6078964652364223,0.6872109247445372,494.0943819140987,0.8062414921965185,0.4885175508538632,
sonar,2.0,280.534,1,0.008790113080792413,0.006075560728734164,0.008793941135604513,0.5027663757107326,0.008786288357280174,0.006409844785829633,0.00530524700027054,59.699458265423424,1.8005189338587992,0.1983999469666345,
sonar,3.0,235.04,0,0.003110558458084321,0.002747604464986592,0.003976961634955198,0.414322259051884,0.0025541275810736863,-0.0017586922582194335,-0.0024019487046078613,55.29428177572339,1.6929144859460152,0.19248688387763896,
sonar,4.0,217.165,0,0.023208008607424925,0.02336049067023427,0.0338126452890678,0.3853278410759623,0.01766709100808889,0.020502085473345238,0.016054533677699222,45.299264755107345,1.9072143573110252,0.1736140254948581,
tae,2.0,21803.3,0,0.007082330773726759,0.0062585814620781674,0.005698393970266422,0.41402853617600893,0.009354110938204796,0.00011396841623356773,-0.0005244138766196055,120.04262044283243,1.0472127358490746,0.3801283934670079,
tae,3.0,16775.4,1,0.02631419215578276,0.02768481835989608,0.02520683048800151,0.36193559274060016,0.02752331954067745,0.00887911245959397,0.013589272548773004,99.66676208871986,1.1042788462657307,0.3374766558094673,
tae,4.0,13221.3,0,0.03816608794552848,0.046005433529489256,0.04188762047955909,0.3111809990024711,0.035051881068158125,0.007994449152107399,0.021593671153922883,96.90851752548882,1.103668339637843,0.34323894977576824,
tae,5.0,10537.7,0,0.04610494002669531,0.06128757875552099,0.0558019051679362,0.2779161092756532,0.039279204038158336,0.014195313697267726,0.02608807653252143,99.86594938807349,0.9866865681764868,0.3643123596056097,
thy,2.0,41608.0,0,0.12763266883059027,0.09664086778750196,0.11764200143753492,0.5372099535501407,0.13947771983801716,0.04775157335177057,0.12215081309750993,115.04657594115812,1.0656984721770706,0.3462207447643411,
thy,3.0,28560.2,1,0.494516046705662,0.3986646698203863,0.4852989292607485,0.8062522135438603,0.5040900576587282,0.5790671581240897,0.4882857152795125,131.83643925618364,0.9235777813115492,0.4565740832904506,
thy,4.0,20082.7,0,0.32113789026291656,0.3032556869761809,0.3691565150432791,0.6175825442367808,0.2841735594981179,0.28141790702370056,0.31003058020629953,154.09183040925103,0.8249080653270541,0.4107051556699643,
thy,5.0,15402.5,0,0.3311263808530725,0.3542028607238399,0.431175075352974,0.5803410290976675,0.26876327890075924,0.27540219092256607,0.31814923898444103,165.92420027947995,0.8300573416438102,0.3944580789974783,
wine,2.0,4543750.0,0,0.42591862667461133,0.3629524368591491,0.3341985166219701,0.6590510206234098,0.5870270068589549,0.3694075388574537,0.4220526675739517,19.490035043004056,2.176493391527314,0.11398383288099236,
wine,3.0,2370690.0,1,0.4287568597645354,0.4657066646034707,0.4288123199785647,0.5835370218944976,0.42870141389448585,0.3711137182308475,0.4226866642766121,18.63851467577729,4.303568871252974,0.04061424616406595,
wine,4.0,1331900.0,0,0.3884332923957888,0.4644628506130969,0.42766704377065773,0.5207343245323419,0.3557931783115363,0.303442531578347,0.3794660493529976,11.956480798763465,7.735705077835789,-0.0318784506667515,
wine,5.0,916379.0,0,0.4109925606542485,0.537739887874978,0.4951389069362355,0.5087079622475457,0.351292227983938,0.3115880103317625,0.4003850916370255,14.735786788755286,5.408027216583188,-0.058420718797688974,
zoo,5.0,158.63,0,0.6993349994752281,1.0984475727336185,0.6629095594628994,0.6806817321677511,0.7399961819075096,0.5811563562389545,0.6707532901380499,82.21871061168216,0.9255466297226398,0.4301899320142995,
zoo,6.0,134.773,0,0.7450441838593459,1.235315542067745,0.7455089365365565,0.7363517316948206,0.7445800102777634,0.6610838742714487,0.7159708514353341,79.97448856682449,0.9310474847925786,0.4477971563030443,
zoo,7.0,119.704,1,0.7816625894813721,1.3471139658020228,0.8129789238768711,0.7741355207962075,0.7526694063540147,0.7087529337715824,0.7527195513185745,76.21779577510424,1.0211302587108235,0.4405712903716864,
zoo,8.0,109.287,0,0.8078200013977627,1.4227394115400198,0.8586186359239372,0.7879450469883381,0.7626964323306963,0.7251155013659698,0.7790454380030649,72.06147916786657,1.0561214365381413,0.442117718340804,
zoo,9.0,100.12899999999999,0,0.8337886459103071,1.5011749300384132,0.90595421779847,0.8072445195129591,0.7722718101398626,0.7471121363080899,0.8062558551394664,69.13282029937969,0.9903091219416648,0.4547490257242741,

